A Tool for Rejuvenating Feature Logging Levels via Git Histories and Degree of Interest

Logging is a significant programming practice. Due to the highly transactional nature of modern software applications, massive amount of logs are generated every day, which may overwhelm developers. Logging information overload can be dangerous to software applications. Using log levels, developers can print the useful information while hiding the verbose logs during software runtime. As software evolves, the log levels of logging statements associated with the surrounding software feature implementation may also need to be altered. Maintaining log levels necessitates a significant amount of manual effort. In this paper, we demonstrate an automated approach that can rejuvenate feature log levels by matching the interest level of developers in the surrounding features. The approach is implemented as an open-source Eclipse plugin, using two external plug-ins (JGit and Mylyn). It was tested on 18 open-source Java projects consisting of ~3 million lines of code and ~4K log statements. Our tool successfully analyzes 99.22% of logging statements, increases log level distributions by ~20%, and increases the focus of logs in bug fix contexts ~83% of the time. For further details, interested readers can watch our demonstration video (https://www.youtube.com/watch?v=qIULoAXoDv4).

==> Makefile <==
PAPER=paper
all:
	latexmk -pdf -shell-escape $(PAPER)
automated:
	latexmk -pdf -shell-escape -interaction=nonstopmode $(PAPER)
continuous:
	latexmk -pdf -pvc -shell-escape $(PAPER)
preview: all
	gio open $(PAPER).pdf
clean:
	latexmk -C $(PAPER)
	rm -rf _minted-*
	rm -f *.aux *.log *.bbl *.blg *.dvi *.synctex.gz *.out *.fdb_latexmk \
		*.fls *.nav *.toc *.snm *.spl *.vtc *.pyg *.vrb *.bcf *.run.xml *.tdo \
		*-blx.bib
	rm -rf $(PAPER)
test: automated check
check:
	chktex -xH -n 6 $(PAPER).tex 2> /dev/null | tee lint.out
html: all
	rm -rf $(PAPER)/
	latex2html -split 0 $(PAPER)
	gio open $(PAPER)/index.html


==> abstract.old.tex <==
\begin{abstract}

that ``rejuvenates'' log statement levels based on how ``interesting'' the enclosing methods are to the developers.

We hypothesize that portions of a system that are worked on more and more recently should have higher log levels (e.g., INFO as compared to FINEST) and vice-versa.

This places event logs related to tasks that are currently more important to the forefront while pushing event logs related to tasks worked on in the past to the background. The goal is to reduce information overload, bring more relevant events to developers' attention, and alleviate developers from manually making log level changes.

The transformation decision is made by analyzing the ``degree of interest'' (DOI) values of enclosing methods for logging invocations. DOI value is a kind of real number for a program element which shows how developers are interested in it. It is computed from the interaction events between developer and element, such as developer edits the element. In this project, we compute the DOI using the project's git history.

\end{abstract}


==> acknow.tex <==
% use section* for acknowledgment
\section*{Acknowledgments}

Support for this project was provided by PSC-CUNY Awards \#617930049 and \#638010051, jointly funded by The Professional Staff Congress and The City University of New York.

==> approach.tex <==
% chktex-file 17
\section{Approach}\label{sec:approach}

\subsection{Overview}

\begin{figure*}
	\centering
	\includegraphics[scale=0.45]{flowchart}
	\caption{Logging Level rejuvenation approach overview.}\label{fig:overview}
\end{figure*}

We detail an automated approach that programmatically manipulates a Mylyn DOI model~\cite{Kersten2005} using git histories to evolve event logging statement levels to better align with the current software features of interest. While this section focuses on concepts, \cref{sec:impl} describes our implementation. \Cref{fig:overview} depicts a high-level overview of the approach. Mylyn~\cite{Kersten2006} has been traditionally used to track and associate edit and graphical selection events in an IDE to a particular \emph{task} for which the developer is working. Its main objective is to support \emph{context switching} between tasks. In this paper, however, we use this model to track the ``interest'' of code elements surrounding logging statements (step 4) to find \emph{mismatches} (step 7) between log levels and feature interests for certain kinds of logging statements. Furthermore, to aggregate interest levels across a development team, edits are extracted from git histories (step 3) rather than from interactions with the IDE\@. The DOI model is then programmatically manipulated using the extracted edits (step 5). The final model is then partitioned (step 6) and compared to current logging statement (step 1) levels (step 2). If a mismatch is found, the level is transformed in the source code (step 9). The transformation is guided by a set of heuristics that we define (step 8). The heuristics help identify logging statements that may benefit from the approach and are largely a result of first-hand developer interactions as part of the evaluation in \cref{sec:pulls}. The following subsections describe the approach in more detail.\todoRK{May want to talk about these steps in order.}

\subsection{Logging Statement Level Extraction}

Input to our approach is a set of projects (q.v.~\cref{fig:overview}). Logging statements are extracted from the project (step 1). They are later used for correlating the interest level of surrounding code when finding mismatches (step 7), applying heuristics (step 8), and as possible transformation sites (step 9). From the statements, the current levels are extracted (step 2), which is later used for mismatch identification (step 7). This is performed in two different ways, depending on the kind of API being used. For instance, in JUL, logging methods come in two flavors, namely, convenience APIs and standard APIs. Convenience APIs have method names that correspond to the desired log level (e.g., line~\ref{lne:logOldTemp}, \cref{lst:wombat}). Standard APIs, on the other hand, are ones where the logging level is passed as a parameter (e.g., line~\ref{lne:logTemp}, \cref{lst:wombat}). In both cases, we extract Abstract Syntax Trees (ASTs) from the underlying source code. While the convenience case is straight-forward, in the standard case, our current implementation (\cref{sec:impl}) only extracts levels from parameters that are passed literal values. While using data-flow analysis to more accurately extract levels stored in variables is a subject of future work, despite this limitation, we were able to successfully \analyzedPercentage\ of logging statements during our experiments (\cref{sec:eval}).

\subsection{Mylyn DOI Model Manipulation}\label{sec:mylyn}

\subsubsection{Background}\label{sec:mylyn:background}

The Mylyn Eclipse IDE plug-in maintains focused contexts of entities relevant to a particular task using a Degree of Interest (DOI) model. A context is comprised of the relevant elements (e.g., classes, methods, fields), along with information pertaining to how \emph{interesting} the elements are to the related task. The more a developer \emph{interacts} with an element (e.g., navigates to a file, edits a file) when working on a task, the more interesting the element is deemed to be, and vice-versa. There is also a notion of \emph{decay}, i.e., as other elements increase in DOI, elements that were once ``interesting'' decrease in DOI\@. Mylyn then alters the behavior of the Eclipse workbench such that only interesting elements are displayed throughout the various workbench views.

% At the beginning of research, we were utilizing the Mylyn task context to ascertain the interest levels of logging statements. However, we found that many developers did not use Mylyn and their projects did not have any task context, so that we cannot read DOI values through Mylyn. Furthermore, we expect our tool could help different developers at project level rather than workspace level. The log level changes that our approach will suggest to developers will possibly affect multiple developers in that they will accept the log levels change when they pull from the repository, i.e., the developer uses our approach (plug-in), possibly accepts some or all of the changes, and commits the results. Other developers will pull and have the new log levels appear in their own (local) repositories. This is to say that the changes assisted by our approach are global at the project level, i.e., it affects the entire project and all of its developers. The local Mylyn task context, however, is confined to the workspace of a single developer. Few developers created global task and shared with other developers. As such, for our approach to be effective, we expanded the Mylyn task context to include events from other developers' workspaces. We did this by using git repository log information as the activities of other developers exist there regardless of whether or not those developers use Mylyn.

\subsubsection{Repository Mining}

In this work, we adapt the Mylyn context to ascertain the interest levels of code surrounding logging statements.
% The Mylyn context, however, currently does not work this way.
Traditionally, Mylyn is used for \emph{context switching}, i.e., Mylyn stores relevant elements in task contexts so that developers may easily switch between tasks without losing their focus on the code elements for which they have been working. It is personal in nature and is confined to the workspace of a single developer.
% In our situation,
However,
% we envision any logging statement level changes to be persisted in the project repository (e.g., in git), which would then propagate the changes to \emph{all} developers.
changes assisted by our approach are \emph{global},
% at the project level,
i.e., they affect the entire project and all of its developers. As such, for our approach to be effective, we conceptually expand the Mylyn context to include interests from all developers by mining git repository log information (step 3; our implementation uses JGit~\cite{EclipseFoundation2020b}).
% as the activities of other developers exist there regardless of whether or not those developers use Mylyn.
%%%%%%%%%%%%%%%%%%%%
% \subsection{Tasks}
% \citet{Kersten2006} heavily relies on the notion of tasks. In other words, DOI values are highly tied to tasks. If a developer is working on a particular task, code elements in their project have a particular value tied to that particular test. Once they switch tasks, which is a central notion in their work, the DOI values associated with the project may change. The tasks store what's called a \emph{context}, i.e., DOI values are per context. In our situation, however, we making code transformations that will \emph{persist} among all tasks. As such, we need to somehow aggregate the DOI values in all task contexts. We do this by average the DOI values across tasks.
%
% For example, a developer may be working on a task, in which case the enclosing method of a log statement has a DOI value of 5. Now, when they switch tasks to say a new task, i.e., one that has no history of work, the DOI value for that same method will not dip to 0. We should take this into account because it could be an indication that that particular log statement is no longer of interest to the developer. In this case, our approach will average the DOI value associated with the logging, resulting in a value of 2.5 (no related work and future work).
%%%%%%%%%%%%%%%%%%%%
% \paragraph{Merge Commits}
Merge commits are not processed due to possible duplication among the multiple parent commits. However,
% we found in our experiments that
such commits typically do not make up a large portion of commits.

% There's a chance that we will process multiple parents of the merge commit, which may be repetitive depending on whether there was a conflict resolution.

% There's an issue with our approach regarding merge commits. We don't process them to avoid repetitive processing. However, this could cause our approach to miss new code that resulted from resolving merge conflicts. The changes in merge commits are arbitrary, though they are supposed to be for resolving conflicts.

% Currently, we don't process merge commits to avoid repetitive processing. Merge commits without conflicts should be easily ignored, but merge commits with conflicts could cause duplicate changes. Moreover, merge commits with conflicts don't account for a large percentage in the all merge commits. We evaluated the subject \javainline{htm}, and found that only 31 of 341 merge commits include conflicts, i.e., most of merge commits do not have conflicts which should be evaluated by our tool. However, ignoring merge commits could cause our approach to miss new code that resulted from resolving merge conflicts. The changes in merge commits are arbitrary, though they are supposed to be for resolving conflicts.

% \subsubsection{Git commits processing}

% We process the commits as follows:

% \begin{verbatim}
% for each commit in the current branch.
% 	// normal commits
% 	if |parents(curr)| = 1
% 		process(curr, parent)
% 	// special case when we're at the initial commit.
% 	if |parents(curr)| = 0
% 		process(curr, NIL)
% \end{verbatim}

% \javainline{process()} is a method to extract method changes in Git diff. The first commit is special, because we cannot compare it and its parent to get diff. For the commits with one parent, we get the diffs between it and its parent. Then, we apply our change detection algorithm on is to extract method changes.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTE: This may be interesting to discuss in a tool paper.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This activity of the work presented here can also be used as a more general Mylyn utility to incorporate VCS information into the Mylyn context and actually solves \href{https://bugs.eclipse.org/bugs/show_bug.cgi?id=433030}{this bug}. That bug, though, only considers adding a single commit (diff) to the Mylyn context (also see \url{https://www.eclipse.org/forums/index.php/t/699154/}). Here, however, we create ``interaction events'' out of a \emph{history} of commits in the project.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Enhancing the DOI Manipulation Model}

% We would file to use our approach without a Mylyn task being activated. When the task is activated, Mylyn will record UI interaction events. But, not everyone uses Mylyn, which tracks UI events. So, we would like to retroactively build element DOIs. But, many projects use version control like git. As such, we support version control (git) events as DOI manipulation.

% We would like to use our approach without an existing non-empty Mylyn task context. When the task is activated, Mylyn will record UI interaction events. But, not everyone uses Mylyn, which tracks UI events. So, we would like to retroactively build element DOIs. But, many projects use version control system like Git. As such, we support version control (Git) events as DOI manipulation.

% The easiest thing to do would have been to analyze the Git history and determine which files are edited and increase the DOI values of those files. The solution works if compilation unit (file) increases in DOI would have implicitly propagated to constituent elements of the file, however, that was not the case. Moreover, our focus is on the logging statements not the files. As such, 

% The easiest thing to do would have been to analyze the git history and determine which files are edited and increase the DOI of those files. But, our focus is on the logging statements not the files. We were curious if compilation unit (file) increases in DOI would have implicitly propagated to constituent elements of the file, however, that was not the case. As such, we extracted enclosing methods of changes in the git history and bumped the DOI of those methods.

\subsubsection{Converting Code Changes to Interaction Events}\label{sec:convert}

As noted in \cref{sec:mylyn:background}, a central notion of Mylyn are ``interaction events,'' which dictate how the DOI model is manipulated. The more interaction a particular element has, the larger its DOI and vice-versa. Although Mylyn has a broad spectrum of different kinds of interaction events, our work focuses on ``edit'' events as we are mining code changes in git repositories. % chktex 38
% Mylyn also has a broad array of different kinds of (non-code-related) IDE elements (e.g., files, projects) that are associated with interaction events. Since we are dealing with code surrounding logging statements, we are only interested in creating edit events related to \emph{code} elements. Unfortunately, the smallest unit of code element granularity in the current Mylyn implementation is method declarations. In the future, we plan to extend Mylyn to accept finer a granularity of code, such as blocks.

In converting code changes in git to Mylyn interaction events to discover ``interesting'' code surrounding logging statements (step 4), we
% process the following types of edits:
mainly focus on code changes to method (and ctor) bodies.
% We extracted changes of enclosing methods in the Git history and bumped the DOI of those methods. Every method will receive a DOI value. In our future work, we would like to choose more software parts, such as adjacent statements, enclosing block etc.
While edits to other kinds of code elements, e.g., fields, could be in close proximity to logging statements, this is currently not supported and does represent a popular use case.\todoRK{Why is this not supported?}
% We use Git edit differences to extract method changes. Another methodology that we did not pick is to use AST~\cite{ast} differences. There are three reasons that we choose edit differences. First, it is more effective than using AST differences, because comparing all AST nodes is computationally expensive. Second, our tool is trying to imitate mylyn plugin, i.e., it considers the non-code changes, such as whitespace, but using AST differences will ignore those non-code changes. Third, we could get git edits from git diffs easily, but it is time-consuming and difficult to get AST differences for all git diffs.
Furthermore, git edits were parsed to extract changes, as opposed to AST differencing, which can be computationally expensive. Moreover, AST differencing does not include whitespace changes, which are desirable in this situation as they are traditionally considered by Mylyn. Once interaction events have been created, they are processed by Mylyn just as if they had emanated from the IDE (step 5).

% \subsubsection{Detected Changes}

% We convert the following edits into interaction events:

% Given git diffs, we could extract four kinds of method changes from the Git edits in them:

% \begin{enumerate}

% 	\item Code changes to method bodies.

% 	\item Method parameter changes.

% 	\item Method name changes.\label{itm:methodname}

% 	\item Adding a method.

% 	\item Javadoc changes to methods.

% \end{enumerate}

% Each of these kinds of changes in the Git history will cause interaction events of the kind EDIT to be produced in our approach. For~\cref{itm:methodname}, we use a refactoring detection approach as described below to find the new name of the method to incorporate into the interaction event.

% \subsubsection{Method changes extraction}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=8cm]{set_difference}}
% \caption{Flow chart for our tool.}\label{set} %TODO: This isn't a flowchart.
% \end{figure}

% Our algorithm is based on the set difference (Figure\ref{set}) and looking for the mappings from two sets A and B. The set A is composed of all method signatures in edits of revision A (old version), while the set B is all method signatures in revision B (new version). The reason that we select the method signature as the element of the set is that the method signature could uniquely identify the method. The difference set A-B contains all methods which will be renamed, deleted or whose parameters could be modified (the number of parameters or the parameter types are changed). The difference set B-A contains all methods which were renamed, added or whose parameter types are changed. The intersection set contains all methods only with method body changes or parameter renaming. First, the algorithm checks the intersection set to get the method changes where method signatures keep same. Then, for each method in A-B, if its corresponding method could be detected in B-A, it experienced renaming or parameter changes. Otherwise, it is a new method which is deleted by the developer in this commit. The remaining elements in B-A are added method signatures. The algorithm to get the mapping from A-B to B-A is based on method signature comparison and method similarity check.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTE: This is for a tool paper:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Interaction events}

% Our tool converts each method change to an interaction event with Kind EDIT sequentially. Then, Mylyn could compute DOI values for all methods. For a common task context, it could be built from different kinds of interaction events, such as SELECTION, etc. However, Git commits cannot store as much information as we need, we have to miss some information. In the future, we would like to integrate existing Mylyn task context with the simulative task context that we build from Git history. In this case, we will hold enough information.

% Mylyn treats negative DOI values as uninteresting. The view ``Focus on Active Task'' in Eclipse only shows elements with positive DOI values. The elements with negative DOI values are treated the same by Mylyn. Our tool could produce negative DOI values. If an element in active context are not accessed indirectly or directly for a long time, it will experience multiple times of decay and its DOI values could become negative. Thus, our processing regards negative DOI values as 0. The minimum DOI value is 0.

% See issue here: https://github.com/ponder-lab/Logging-Level-Evolution-Plugin/issues/111
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Rename Refactorings}

% The situation that our tool works is that Mylyn works on a version of files (usually the latest version), and our tool could analyze all Git commits before that file version to bump DOI values of methods in the version that Mylyn works on.
% The issue is that the
% Historical
Program elements (e.g., methods) changed in the git commit history may no longer exist in current project version where log level transformations would take place.
% the Mylyn working version, that is why we need to detect method refactoring. Given a historical method, we need to know its latest method in the Mylyn working version.
Such historical elements that were removed from the project are ignored as they are not in the input project version. However, elements that have underwent rename refactorings do need to be considered as they will have a counterpart in the current version.
% There are two-level refactorings which could cause changes of method signatures:
% \begin{itemize}
% 	\item File-level refactoring: file renaming or file copy.
% 	\item Method-level refactoring: method renaming, method parameter modification.
% \end{itemize}
% \paragraph{Move Refactorings}
% Git records move operations between files (like rename a file etc.). We process these changes from Git accordingly.
%TODO: how can we process copying?? (ignoreing for now)
% \paragraph{Rename Refactorings}
% This is about renaming methods. We track the renames using existing work (TBD), we build a tree of changes,
To this end, during git repository mining, we maintain a data structure that associates rename relationships between program elements, e.g., method signatures. If a code change is discovered during the mining process, before converting it to an interaction event, a lookup is first performed
% on the data structure
to retrieve the changed element's signature in the current version. Unfortunately, dealing with refactorings necessitates two traversals, one to create the renaming data structure and the other to process code changes. However, in our implementation, we have a performance improvement where code changes are cached during the renamings detection, and only the code changes are traversed subsequently rather than the git history.

% Renaming graph stores methods which experience signature changes. It consists of multiple sequences of method signature history. Each sequence is corresponding to a method. We build our renaming graph through file-level change and method-level changes.

% Through renaming graph, we could get the latest method for a historical method in a commit even its method signature has changed before. We use ``latest method'' to describe the methods in the revision that Mylyn works on. While we are evaluating a git history and getting a method change for a historical method in the commit, we could not generate interaction event for it directly. Because this historical method could not exist in the current source code, and Mylyn can only bump DOI values for the methods it could touch. In this case, we need to get the corresponding method at first. Then, we could let Mylyn bump the DOI for it.

% To curtail run time overhead,
Because only rename refactorings are needed, instead of using more advanced approaches~\cite{Tsantalis2018}, our current research prototype uses lightweight approximations, such as basic method signature and body similarity comparison, for rename refactoring detection. Nevertheless, during our experiments, we were able to successfully analyze the change history of code surrounding \logs\ logging statements across \NumProjects\ projects. In the future, we plan on exploring integrating (at least parts of) such techniques for improved accuracy.

\subsection{DOI-Log Level Association}

The result of Mylyn processing all of the generated interaction events as part of step 5 is a rich (depending on the amount of git history available) DOI model where the most and most recently edited code is associated with the highest DOI and vice-versa. The DOI values (a real non-negative number) from the final model are then partitioned so that DOI ranges can be associated with levels from the underlying logging framework (step 6). The association is then used in the next step (step 7) to discover mismatches between interest and logging levels for a certain class of logging statements (as guided by heuristics in step 8).

% If developers do not select any log category, the DOI range of the evaluated project will be divided into 7 partitions equally. The DOI intervals from low DOI value to high DOI value will be corresponding to \javainline{FINEST}, \javainline{FINER}, \javainline{FINE}, \javainline{CONFIG}, \javainline{INFO}, \javainline{WARNING} and \javainline{SEVERE} respectively. If developer select log category, the DOI range will be divided into 6 partitions. \javainline{CONFIG} will be excluded. However, for the log category (\javainline{CONFIG}/\javainline{WARNING}/\javainline{SEVERE}), we do not transform the log levels in the enclosing methods with the DOI value which is in the DOI interval for \javainline{CONFIG}/\javainline{WARNING}/\javainline{SEVERE}, and we do not transform \javainline{CONFIG}/\javainline{WARNING}/\javainline{SEVERE} either, i.e., two different log categories could produce the same DOI intervals for the same project with the same git history, but their transformation strategies are different, which could result in different transformation results.

Conceptually, the partitions are created by subtracting the highest DOI value in the model by the lowest and dividing the result by the number of different logging levels the logging framework provides. This calculation produces the partition DOI range size. Then, each DOI range is associated with the level by order. For example, the least logging level (e.g., \ji{FINEST}) is associated with the first partition (e.g., with DOI range $[0,2.54)$). However, one of the heuristics (q.v.~\cref{sec:heuristics}) allows developers to choose whether or not to consider particular levels (e.g., they may choose to treat \ji{WARNING} and \ji{SEVERE} as kinds of log \emph{categories} rather than levels), and this can influence the partitioning scheme. In such cases, certain partitions will purposely not cause mismatches to be detected, thus affecting the transformations performed. Once the partitions have been formed, potential mismatches are discovered (step 7) by comparing the partitions with the current logging statement levels from step 2. % FIXME: How is surrounding code identified? chktex 9
If a mismatch is found, the statement is considered for potential transformation subject to the heuristics outlined next.

% After we bump DOI values for all methods, we could read DOI values for them through Mylyn. Based on our assumption, we would like to see higher levels in the enclosing methods with higher DOI values, and vice versa. Then, we build a transformation model. In this model, a mapping between DOI interval and log level is introduced.\todo[inline]{RK\@: Need to discuss boundaries.} We divide our DOI value ranges equally into several categories and the number of categories is same as the number of possible log levels that our tool may transform to, i.e., each DOI values interval is corresponding to a target log level. For a log invocation, our tool rejuvenates its log level by computing which DOI value interval its DOI value of the enclosing method falls in.
%
% There are two kinds of enclosing methods with 0 DOI value. One is the method never analyzed before.Our tool doesn't consider it. We cannot judge it without knowing its history. The other is the method which is analyzed before but its analysis is in a very earliest commit. Its decay becomes 0 because of decay. Our tool does consider it.

\subsection{Heuristics}\label{sec:heuristics} % FIXME: Are these ad hoc?

Log level transformations are guided by a set of heuristics (step 8). In our implementation (\cref{sec:impl}), these are manifested as tool options.
% in the GUI\@.
The heuristics were largely formulated during our pull (patch) request study (\cref{sec:pulls}) where we had first-hand discussions with contributors of large and popular open source projects. The main purpose of the heuristics is to help identify the kinds of transformations that may yield useful results. For instance, the heuristics are used to avoid undesirably transforming the logging statements on lines~\ref{lne:tempWarn},~\ref{lne:invalidInput}, and~\ref{lne:fileError} in \cref{lst:wombat4}.

The heuristics utilized include the following:

\begin{enumerate}

	\item Treat particular levels as log categories.\label{itm:CWS}

	\item Never lower the level of logging statements appearing within catch blocks.\label{itm:catch}

	\item Never lower the level of logging statements immediately following if statements.\footnote{\mintinline[fontsize=auto]{java}{else} is treated similarity.}\label{itm:followingifs}

	\item Never change the level of logging statements immediately following if statements whose if condition contains a log level.\label{itm:wrapping}

	\item Never lower the level of logging statements \emph{having} particular keywords in their log messages.\label{itm:withkeys}

	\item Never raise the level of logging statements \emph{without} particular keywords in their log messages.\label{itm:withoutkeys}

	\item Only consistently transform the level of logging statements appearing in overriding methods.\label{itm:subtyping}

	\item Only transform the level of logging statements up to a transformation distance threshold.\label{itm:threshold}

\end{enumerate}

For~\cref{itm:CWS}, a developer may choose to treat \ji{WARNING} and \ji{SEVERE}\footnote{These levels vary depending on the logging framework used in our implementation.} as logging statement categories rather than traditional levels. This way, developers can denote that logging statements with such levels have special semantics other than a sliding scale. Denoting \ji{WARNING} and \ji{SEVERE} as logging level categories can be used to avoid transforming the statements at lines~\ref{lne:tempWarn} and~\ref{lne:fileError} (but not line~\ref{lne:invalidInput}) of \cref{lst:wombat4}.

% Log level may not all be similar. For example, while INFO--FINEST could be ``sliding'' levels, i.e., their output should be controlled by the level of verbosity needed, other levels may be persistent. For example, \javainline{CONFIG} (\url{http://docs.oracle.com/javase/10/docs/api/java/util/logging/Level.html#CONFIG}) is more dependent on the content of the log message itself. These log levels correspond more to log ``categories.'' We allow users to our tool to let us know which levels should be treated as categories and not traditional levels. In such cases, we don't transform these levels because they aren't ``sliding'' levels. By default, we exclude \javainline{CONFIG}. % chktex 8

% The log categories users could choose:
% \begin{enumerate}
% 	\item Traditional log levels.
% 	\item Treat CONFIG as a log category.
% 	\item Treat CONFIG/WARNING/SEVERE as a log category.
% \end{enumerate}

The motivation behind \cref{itm:catch} is that logging statements appearing in catch blocks may serve as notifications of errors rather than more general events.
% As such, we never want to reduce the level of such statements (only increase or leave as-is).
This heuristic ensures that the level of such statements is never reduced. The statement at line~\ref{lne:fileError}, \cref{lst:wombat4} is a prime example as it did not have its level lowered despite the lowering of a level of a nearby statement at line~\ref{lne:fileDecrease} due to recent non-local edits.
% See \url{https://github.com/ponder-lab/Logging-Level-Evolution-Plugin/issues/136}.
The rationale of \cref{itm:followingifs} is similar to that of \cref{itm:catch}, with a prime example being the statement at line~\ref{lne:tempWarn}, \cref{lst:wombat4}.
% See \url{https://github.com/ponder-lab/Logging-Level-Evolution-Plugin/issues/198}.
% We only avoid ``guarded commands'' i.e., if statements having no else clauses.
Below is a real-world example found in \blueocean~\cite{McDonald2018},
% . In this context, the
where two similar logging statements
% are similar although one
appear in each different context:
% is in a catch block, while the other is immediately following an if statement:
% In both cases, we do not want to lower the levels as they portray important events.

\begin{javacode*}{fontsize=\footnotesize,linenos=false}
	try {
		node = execution.getNode(action.getUpstreamNodeId());
	} catch (IOException e) {
		LOGGER.warning("Could not retrieve upstream node: " + e);
		continue;
	}
	if (node == null) {
		LOGGER.warning("Could not retrieve upstream node (null)");
		continue;
	}
\end{javacode*}

% See \url{https://github.com/ponder-lab/Logging-Level-Evolution-Plugin/issues/147}.
\Cref{itm:wrapping} is to prevent logging semantics violations when logging statements are redundantly guarded by run time level checks. We found one real-world example of this in \guava~\cite{Decker2014} during our experiments (\cref{sec:eval}):

\begin{javacode*}{fontsize=\footnotesize,linenos=false}
 if (logger.isLoggable(Level.SEVERE)) {
	logger.log(Level.SEVERE, message(context), exception);
 }
\end{javacode*}

\noindent Altering the level of the logging statement here without also changing the if condition would be counterproductive. A more sophisticated analysis would be necessary to handle such cases, which did not seem typical in our experiments. Moreover, other approaches~\citet{Li2017a} do not deal with this situation.

We found that \cref{itm:withkeys,itm:withoutkeys} to also be helpful with guiding the directionality of the transformations. The keywords used were obtaining empirically during our experiments as well as derived from developer feedback. Stop gap words were used to maximize coverage. Furthermore, the keywords must appear in the literal parts of the log message construction. Keywords for \cref{itm:withkeys} include, ``fail,'' ``disabl,'' ``error,'' and ``exception;'' keywords for \cref{itm:withoutkeys} include ``stop,'' ``shut,'' ``kill,'' ``dead,'' and ``not alive.'' \Cref{itm:withoutkeys} only applies for target levels \ji{WARNING} or \ji{SEVERE}, which are typically used in more critical situations, and does apply when \cref{itm:CWS} is enabled as these will never be target levels in this case.

% \subsubsection{Transformations and Method Overriding}
%
% Log invocations may exist in an overriding method and its overridden method at the same time. For maintaining the substitutability of the evaluated project, our tool will transform the log levels in the overridden method if needed and adjust the levels in the overriding method to make their target levels consistent with the target levels in the overridden method.
%
% The real projects have more complicate cases than the case above. For example, an overridden method could be an overriding method that overrides another method. Considering these kinds of cases, RootDefs~\cite{Khatchadourian2017} is defined to solve the inconsistent level transformations among overridden and overriding methods.
%
% \begin{dfn}
%     $\mathit{RootDefs}(M)$ = \{M' | M overrides M', and M' doesn't override any method\}
% \end{dfn}
%
% Given the definition, a method M could have more than one overridden methods M' in its RootDefs set. Regarding this case, the tool can make a majority vote on target log levels. The most target log level in the RootDefs will be the final target level. Then, our tool will transform all log levels in M and its overridden methods into the target log level we choose.

\Cref{itm:subtyping} was also discovered during our pull request study and emanated from developer feedback. It applies to situations where mismatches are found in both overriding and overridden methods. Specifically, if method $M'$ overrides method $M$ and both $M$ and $M'$ include level mismatches, the transformation target levels in these methods should be consistent. This preserves a behavioral subtyping-like relationship w.r.t.~logging in the methods. Lastly, \cref{itm:threshold} also emerged from developer feedback. As our tool is able to make widespread changes, some developers preferred to curtail the level degree of the suggested transformations. Finally, all mismatches that pass the enabled heuristics are transformed via AST node replacements (step 9).

% \subsection{Transformation}

% \subsubsection{When to do the transformation}

% Do we do it at the discretion of the developer or automatically when they close and open task?


==> background.tex <==
\section{Background}\label{sec:background}

\todoRKi{This should be in \cref{sec:approach}.}

\subsection{Eclipse Mylyn plugin}

\todoRKi{This section title is too technology-specific. You would never have this in a conference paper. It is fine for a tool paper.}

Our research approach reads DOI values of program elements through Mylyn. Mylyn is a task and application lifecycle management plugin in Eclipse~\cite{mylynK}. It assigns a real number to each program element (a method, a source file etc.) by evaluation of interaction events during an active task period. That real number is a representation of degree of developers' interests, and is named as ``DOI value''. Developers create a Mylyn task. They can add modify the task title and  When the task is active, all interaction events between developers and program elements could be recorded by Mylyn.

The sort of interaction events~\cite{mylyn} are listed below:
\begin{itemize}
  \item Selection: user select elements
  \item Edit: edit text in the editor
  \item Command: commands and actions invoked via buttons, menus, and keyboard shortcuts
  \item Preference: workbench preference changes
  \item Prediction: elements determined by Active Search
  \item Propagation: elements determined to be structurally related
  \item Manipulation: operation on DOI directly
  \item Attention: interaction with a task, used for the meta-context.

\end{itemize}

Mylyn drives task context from the sequence of interaction events~\cite{Kersten2006}. Task context is a graph whose elements are program elements and the edges are the relationships of elements. 

\subsection{DOI model}

DOI model is core model of Mylyn. The Mylyn's DOI model describes the interests of the code elements which are relevant to the task at hand~\cite{Kh2017}. DOI value does not only represents how developers pay attention to a program element frequently, but also show how they focus on the element recently. DOI model is a balancing model. When it increases the DOI value of a program elements through analyzing an interaction event, it could decrease the DOI value of other program elements which are not involved by the event in the task context. The operation for decreasing DOI value is named ``decay''. 

DOI values are highly tied to tasks. Each event in the task context could affect the DOI values for relevant Java code elements. The DOI value could change after the developers switch tasks, e.g.,  if a developer is working on a particular task, code elements in their project have a particular value tied to that particular test. Once they switch tasks, which is a central notion in their work, the DOI values associated with the project may change.

\subsection{Git and JGit}

%todo: what is commit
%todo: what is diff

Git is an open-source distributed version control system~\cite{git}. Git takes a picture on the files it tracks if these files have some changes. Each time developers modify file, they could make a commit and pushed the commit to the remote repository. A commit is used to store file changes for a certain version. It has its index (sha-1) to unqiuely identify itself. It also has a timestamp for the time when it is pushed. A commit has two revisions of files. One revision is old revision before modifications, the other one is new revision after modifications. Diff is file differences between two revisions of files, so the diff of a commit is the file differences between the old and new revisions. In each file, diffs for a file are composed of several hunk. Hunk is a pair of text blocks. One text block is the text deleted in first revision of file, and the other of them is the text added in the second revision of file. The hunk shows a text block change in a file. Hunk is not the samllest unit for file differences. Each hunk could contain several edits. Edit is similar as hunk, but it is always small.


JGit is a lightweight Java library of Git version control system. Developers could access repositories, read git commits and so on through Java APIs it provides. JGit stores diffs at file level. Each file diff is store in \javainline{DiffEntry}. Every object of \javainline{DiffEntry} has its type of changes. All types of changes are following~\cite{jgitChangeType}:

\begin{itemize}
  \item ADD\@: a file addition.
  \item DELETE\@: a file deletion.
  \item COPY\@: a file copy and keep the original one. 
  \item RENAME\@: a file rename.
  \item MODIFY\@: a file content or mode modification.
\end{itemize}


==> content_old.tex <==
\commentRK{Please model the content after \url{https://bit.ly/3clv2fo}.}

\input{intro}

\commentRK{As discussed, there should be a section corresponding to each bullet point in the CfP. The next section should be about ``the software testing and analysis challenge(s) the tool addresses.'' Our focus is on analysis challenges. What are the analysis challenges the developers face in this domain? How does the tool help \emph{address} those challenges? This section should be modeled after \url{https://bit.ly/2zcovFz}, which was modeled after the original motivation section of the conference paper.} % chktex 36

\input{motive}
\input{user}
\input{impl}
%\input{approach}
%\input{eval}
\input{related}
\input{eval}
\input{conc}
%\input{acknow}


==> eval.tex <==
\section{Evaluation}\label{sec:eval}

We evaluated on \NumProjects\ Java projects having \MLOC\ million lines of code and \logsThousands\ log statements. Our tool was able to successfully analyze \analyzedPercentage\ of logging statements, increase the distribution of log levels by \distributionPercentageIncrease, and identify logs that were manually changed with a recall of \recall\ and a precision of \precision\ with a level direction match success rate of \levelDirectionSuccessRate. Furthermore, we analyzed git histories for bug and non-bug fixes with nearby feature logging statements from 12 subjects and increases the focus of logging code in bug context \logInBugContext\ of time. Moreover, two of our pull (patch) requests were integrated into large and popular open-source projects, namely, \jenkins~\cite{pr-for-jenkins} and \selenium~\cite{pr-for-selenium-new}.\commentRK{References to these?}


% % Research questions example: What is the best way to distribute log level intervals? Equal? Weighted (which is more popular)? Which one works the best?

% \subsection{Implementation}\label{sec:impl}

% Our approach was implemented as a publicly available, open source Eclipse IDE~\cite{EclipseFoundation2020a} plug-in~\cite{Tang2020} and built upon JGit~\cite{EclipseFoundation2020b} and Mylyn~\cite{EclipseFoundation2020}. Eclipse is leveraged for its extensive source-to-source transformation support~\cite{Baeumer2001}
% % and GUI
% and that it is completely open-source for all Java development.\todoRK{Footnote about IntelliJ here.} It also supports popular build systems, so that our plug-in may be applied to projects that use different IDEs. JGit is used for git commit extraction and Mylyn for manipulating and querying a DOI model. For transformation, Eclipse ASTs with source symbol bindings are used as an intermediate program representation. Two popular logging frameworks, namely, \javainline{java.util.logging} (JUL)~\cite{Oracle2018b} and SLF4J~\cite{QOS.ch2019}, are currently supported. However, our implementation can be extended to include others. Heuristics (\cref{sec:heuristics}) are presented as a series of tool options.
% % as part of the transformation wizard GUI\@. Developers may select (or unselect) desired transformations using the wizard or simply allow the tool to make all transformation suggestions and use git to decide which are committed to the repository.
% % It is also possible to run the tool from the command-line.

% % TODO: Do we want to talk about this? The granularity of ``surrounding code'' in our current research prototype is enclosing method declarations.

% \todoRKi{Discuss how we had to alter the original Mylyn decay rate. Mylyn was not originally designed to handle the significant number of typical changes produced in git repositories. Instead, it was originally designed to track changes to the IDE by a single developer. As such, we found that elements in the DOI decayed too rapidly due to the vast amount of input produced by git repository mining.}

% \todoRKi{Discuss how our tool is split into different plug-ins. Mainly, we split the tool into plug-ins that extend the functionality of Mylyn by enabling it to handle git repository changes (this is the mylyngit plugins) and provide the analysis and code transformations (these are the log plug-ins).}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % NOTE: This can be for the tool paper:
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % We build a hash table of mappings a method signature and its ``new'' signature using this tree from the method renaming tree to improve the performance of rename lookups.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % NOTE: This can be for the tool paper:
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \subsubsection{Multiple projects}
% %
% % There is an engineering challenge regarding subprojects and git repositories.
% %
% % For multiple projects, we treat each of them as an independent project and process them sequentially. The task context is cleared after each processing. For every project, we need to traverse its git history, so some Git history in a repository with multiple subprojects may be analyzed more than one time. For eliminating duplicate analysis, memoization is used here. Each time analyzing a project, we store some intermediate data, such as method changes. At the same running time, if the tool analyzes a project with the same repository, it will read the stored data directly. Thus, repository is only processed once for every running time of the tool.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Experimental evaluation}

% The evaluation proceeds in three phases, namely, a quantitative/qualitative investigation, a comparison against manual log level changes, and a pull (patch integration) request study.

% % \subsubsection{Subject Selection}

% % We chose subjects that use java.util.logging.

% \subsubsection{Quantitative Analysis}

% \begin{table*}
% 	% This table is backed by https://docs.google.com/spreadsheets/d/1kfaB3v7NRJwH13OPZR2mb0UspSEf8Zfu3BcGrJ6-JJ0/edit#gid=1403131595.
% 	\caption{Experimental results. 
% 	% \textbf{Kcmts} is thousands of commits analyzed.
% 	% \textbf{$\delta$KLOC} is thousands of git history source lines of code analyzed.
% 	% \textbf{fw} is logging framework.
% 	% \textbf{logs} is sum of candidate logging statements.
% 	% \textbf{fails} is the sum of failures.
% 	% \textbf{trans} is sum of transformed logging statements.	
% 	% \textbf{catch} is sum of log levels not lowered in catch blocks.		
% 	% \textbf{ifs} is sum of log levels not lowered in if statements.		
% 	% \textbf{conds} is sum of log levels not transformed due to if condition.	
% 	% \textbf{keyl} is sum of log levels not lowered due to keywords.
% 	% \textbf{keyr} is sum of log levels not raised without keywords.
% 	% \textbf{inh} is sum of log levels adjusted by inheritance.
% 	% \textbf{$\overline{\mathit{distance}}$} is average transformation distance, followed by its standard deviation.		
% 	% \textbf{$\sigma_{\mathit{before}}$} is standard deviation of old Java Util logging log levels before the transformation.	
% 	% \textbf{$\sigma_{\mathit{after}}$} is standard deviation of new Java Util logging log levels after the transformation.					
% 	% \textbf{lower} is number of lowered log levels.
% 	% \textbf{raise} is number of raised log levels.			
% 	% \textbf{t (m)} is the total processing time in minutes.
% 	}\label{tab:results}
% 		\resizebox{\textwidth}{!}{%
% 			\begin{threeparttable}
% 				\begin{tabular}{lllllllllllllllllllll}
% 					\toprule
% 					subject & HEAD & KLOC & Kcmts & $\delta$KLOC & fw & logs & fails & trans & catch & ifs & conds & keyl & keyr & inh & $\overline{\mathit{distance}}$ & $\sigma_{\mathit{before}}$ & $\sigma_{\mathit{after}}$ & low & raise & t (m) \\
% 					\midrule
% 					bc-java & a66e904 & 701.57 & 6.00 & 1,213.28 & 1 & 56 & 4 & 11 & 5 & 13 & 6 & 16 & 0 & 0 & 2.64 (1.30) & 1.49 & 2.01 & 11 & 0 & 62.78 \\
% 					blueocean\tnote{*} & c3bfac5 & 49.32 & 4.06 & 137.85 & 2 & 109 & 0 & 13 & 11 & 6 & 5 & 57 & 9 & 0 & 1.54 (0.63) & 1.65 & 1.74 & 11 & 2 & 2.93 \\
% 					californium & 5b026ab & 79.35 & 1.00 & 143.53 & 1 & 986 & 0 & 141 & 23 & 123 & 95 & 317 & 176 & 2 & 1.52 (0.73) & N/A & N/A & 118 & 22 & 7.51 \\
% 					CoreNLP & d7356db & 535.07 & 6.00 & 43,686.03 & 2 & 358 & 0 & 146 & 0 & 87 & 21 & 55 & 0 & 0 & 3.10 (1.43) & 1.84 & 2.16 & 146 & 0 & 444.99 \\
% 					deviation\tnote{*} & 88751d6 & 6.52 & 0.08 & 24.81 & 1 & 91 & 0 & 11 & 1 & 7 & 8 & 48 & 3 & 0 & 2.64 (1.23) & 1.69 & 2.07 & 11 & 0 & 0.06 \\
% 					errorprone & 2118ba3 & 164.65 & 3.99 & 517.18 & 1 & 12 & 0 & 1 & 1 & 0 & 1 & 9 & 0 & 0 & 2.00 (0.00) & 1.61 & 1.86 & 1 & 0 & 17.36 \\
% 					guava & 71de406 & 393.69 & 1.00 & 296.52 & 1 & 36 & 0 & 0 & 0 & 0 & 0 & 33 & 0 & 0 & 0.00 (N/A) & 1.52 & 1.52 & 0 & 0 & 29.63 \\
% 					hollow & ff635ee & 68.60 & 0.90 & 158.73 & 1 & 31 & 0 & 6 & 0 & 3 & 0 & 22 & 0 & 0 & 3.50 (1.12) & 1.02 & 1.98 & 5 & 1 & 2.86 \\
% 					IRCT & d67f539 & 42.29 & 0.89 & 193.69 & 1 & 13 & 0 & 6 & 0 & 0 & 0 & 2 & 1 & 0 & 2.00 (1.41) & 1.22 & 1.51 & 6 & 0 & 2.07 \\
% 					JacpFX & 14c2a4c & 24.06 & 0.37 & 121.41 & 1 & 21 & 0 & 2 & 4 & 0 & 7 & 8 & 0 & 0 & 2.50 (1.50) & 1.47 & 1.69 & 2 & 0 & 0.77 \\
% 					jdp\tnote{*} & 515b7e7 & 35.86 & 1.00 &	99.99 & 2 & 799 & 0 & 180 & 17 &	15 & 4 & 84 & 399 &	0 &	1.70 (0.63) & 0.00 & 1.79 & 139 & 41 & 3.18 \\
% 					jenkins & 4f0436a & 160.60 & 1.00 & 25.28 & 1 & 503 & 22 & 60 & 29 & 52 & 54 & 244 & 22 & 0 & 2.17 (1.25) & 1.73 & 1.84 & 58 & 2 & 3.81 \\
% 					jsilhouette & 8de4e64 & 2.35 & 0.03 & 5.52 & 1 & 22 & 0 & 0 & 0 & 8 & 0 & 14 & 0 & 0 & 0.00 (N/A) & 0.00 & 0.00 & 0 & 0 & 0.04 \\
% 					junit5 & 3969585 & 73.59 & 5.98 & 380.61 & 1 & 9 & 2 & 4 & 0 & 0 & 0 & 2 & 0 & 0 & 3.00 (1.00) & 0.00 & 1.67 & 4 & 0 & 75.25 \\
% 					OpenGrok & 0f3b14d & 71.65 & 4.93 & 377.09 & 1 & 592 & 3 & 61 & 44 & 49 & 41 & 353 & 13 & 0 & 2.70 (1.47) & 1.81 & 2.07 & 53 & 8 & 15.20 \\
% 					selenium & a49fb60 & 93.61 & 1.00 & 75.97 & 1 & 94 & 0 & 28 & 5 & 6 & 0 & 48 & 4 & 0 & 2.96 (0.94) & 1.00 & 1.75 & 27 & 1 & 1.45 \\
% 					SpotBugs & ecc7994 & 187.78 & 1.00 & 94.11 & 2 & 96 & 0 & 44 & 2 & 15 & 6 & 26 & 0 & 0 & 1.57 (0.96) & 1.74 & 2.30 & 44 & 0 & 26.59 \\
% 					WALA & b73a0b2 & 202.45 & 1.00 & 235.50 & 2 & 145 & 0 & 39 & 1 & 38 & 0 & 22 & 16 & 1 & 1.41 (0.54) & 0.94 & 0.94 & 38 & 1 & 9.20 \\
% 					Total &  & 2,893.01 & 40.22 & 47,787.09 & 1.28 & 3,973 & 31 & 753 & 143 & 422 & 248 & 1,360 & 643 & 3 & 2.13 (1.23) & 1.75 & 2.05 & 674 & 78 & 705.68 \\
% 					\bottomrule
% 				\end{tabular}%
% 				\begin{tablenotes}
% 					\item[*] blueocean is \blueocean, deviation is \deviation, and jdp is \jdp.
% 				\end{tablenotes}
% 			\end{threeparttable}
% 		}
% \end{table*}

% Our evaluation involved \NumProjects\ open source Java applications and libraries of varying size and domains (\cref{tab:results}). Subjects were also chosen such that they include logging statements using either JUL or SLF4J and have at least one source code change to a method containing a logging statement (i.e., a candidate statements).
% % We make a list of GitHub repositories with logging invocations and recent commits. During the period of subject selections, the number logging invocations is estimated by searching some logging related keywords in GitHub, such as \javainline{Java.Util.Logging}. We prefer to select some large repositories from famous GitHub organizations like Eclipse. However, we also add some small projects into our list to show our tool can work on different projects of varying sizes.
% Column \textbf{HEAD} is SHA-1 of HEAD at analysis time. Column \textbf{KLOC} is the thousands of source lines of code, which ranges from $\sim$6K for \deviation\ to $\sim$535K for \CoreNLP\@. Column \textbf{Kcmts} denotes thousands of commits analyzed, which can significantly affect the number of candidate statements.
% % Usually, the more git commits are analyzed, the more candidate logs are detected if the Git history of the project is long.
% For some subjects with long git histories, such as \errorp, we choose a large number of commits (the entire history for \errorp) to obtain more candidates. For others, a relatively small number of commits was adequate to obtain all logging statements as candidates (e.g., \spotbugs). Column \textbf{$\delta$KLOC} is the thousands of source lines of code differences analyzed from git history. Column \textbf{fw} is the number of logging frameworks detected (two are currently supported), averaging \num{1.28} (some projects use more than one framework).
% % The column \textbf{fw} in row of \textbf{Total} is average number of logging frameworks for all subjects. Our tool could work on two popular Java logging frameworks: \JUL\ and \slf\@.
% Subjects compiled correctly and had identical unit test
% % (XXX; mostly from XXX)
% results (with the exception of one in an earlier tool version; q.v.~\cref{sec:qual}) and compiler warnings before and after the transformation.

% The analysis was executed on an Intel Xeon-E3 with 4 cores and 31GB RAM and a 20 GB maximum heap size. Column \textbf{t (m)} is the total running time in minutes, averaging  \AvgRuntimePerLog\ secs per candidate statement and \AvgRuntimePerKLOCChanged\ secs per thousand lines of code changed ($\delta$KLOC). The running time is highly related to analyzed source lines per commit (\textbf{$\delta$KLOC}/Kcmts),
% % , averaging $\sim$1188.11. The
% with a Pearson correlation coefficient of 0.98 (ranging from -1 to 1; 1 is an exact linear correlation).
% % . The correlation coefficient is used to measure a linear correlation between two variables, ranging from -1 to 1. A correlation coefficient of  exists.
% \CoreNLP, having a particularly long and intricate git history, is an outlier, taking over half of the running time.
% % , which inflates the averages.
% % \footnote{Analyzing the (large) git history of \CoreNLP has been problematic in our other work; it has a long and intricate git history.}
% Moreover, as explained in \cref{sec:convert}, two traversals are necessary to deal with
% % method
% rename refactorings.
% % We also conjecture that the running time is affected by the computation performed to convert git edit changes to interaction events associated with code elements.
% % Despite some of the running times,
% Nonetheless, since our tool is fully-automated, it can conceivably run as part of a nightly build process.

% \paragraph{Log Level Rejuvenation}

% We analyzed \logs\ candidate statements (column \textbf{logs}) across \NumProjects\ subjects,\footnote{\junit\ only has \num{9} candidates because the current version studied in this phase mainly uses custom logging methods. It was included here as its former versions used JUL and are studied in the subsequent phase.} successfully analyzing \analyzedPercentage\ of candidate statements. Column \textbf{fails} indicates the number of times a current logging level was not able to be extracted. Such failures include situations where, for example, the logging level is stored in a variable, necessitating more sophisticated analyses.
% % and where the logging statement is outside of a method context.
% Column \textbf{trans} represents the number of transformed logging statements (\transPercent\ of candidates), which is dependent on the mismatches found and the enabled heuristics.

% For this phase, to more fully understand the effect of the heuristics, all heuristics were enabled with the exception of log categories (\cref{itm:CWS} in \cref{sec:heuristics}) and the transformation distance threshold (\cref{itm:threshold}). To that end, column \textbf{catch} is the sum of levels not lowered due to \cref{itm:catch}, column \textbf{ifs} the sum of levels not lowered due to \cref{itm:followingifs}, and column \textbf{conds} the sum of levels not transformed due to \cref{itm:wrapping}. Column \textbf{keyl} is the sum of log levels not lowered due to keywords (\cref{itm:withkeys}), and column \textbf{keyr} the sum of log levels not raised without keywords (\cref{itm:withoutkeys}). Column \textbf{inh} is the sum of levels not adjusted due to inheritance (\cref{itm:subtyping}).

% To understand the grade of transformations made, column \textbf{$\overline{\mathit{distance}}$} is average transformation distance, followed by its standard deviation. In every logging framework, the distance between two adjacent log levels is 1.
% % The total row in this column is the average. transformation distance for all transformed logging statements followed by its corresponding standard deviation.
% To understand the directionality of the transformations, column \textbf{low} is number of lowered log levels, while column \textbf{raise} is number of log levels raised. The results show that our tool more frequently lowers logging statement levels. This is most likely indicative of the smaller number of features that developers focus on at a particular time in a project. % FIXME: Is this discussion?

% % Logging frameworks offer a wide variety of levels that can help debug programs.
% During the experiment, we found that developers did not always utilize the full spectrum of log levels available. This is evident in column \textbf{$\sigma_{\mathit{before}}$}, which is the standard deviation of log levels for \emph{before} any transformations,\footnote{Only includes JUL, which accounted for the majority of subjects. N/A indicates that JUL was not used.} averaging only \distributionBefore. Column \textbf{$\sigma_{\mathit{after}}$}, on the other hand, is standard deviation \emph{after} transformation, averaging \distributionAfter. The \distributionPercentageIncrease\ increase indicates that our approach can improve log level diversity, allowing developers to take more of an advantage of the expressiveness that logging frameworks offer.

% \subsubsection{Qualitative Analysis}\label{sec:qual}

% \todoRKi{Can use more discussion here.}

% % Some projects, e.g., jetty, wrap the logging API\@. Developers set log level in purpose to match their if condition. These cases do not apply to our previous transformations through analysis of DOI values, because transformations may break developers' logic. Thus, regarding the cases, our approach doesn't transform a log level if there exists an immediate if statement whose condition contains a log level. We assume that if the log statement is ``guarded'' by an if condition mentioning a log level, there must be some correlation between their log levels.

% % Regarding our setting for not reducing the level of log statements within catch blocks, in our empirical study, we found three log level changes that appeared in catch blocks\todo{That's for an old version of the tool. Should we still mention this?}\todoRK{Probably not}. Indeed, in one project (IRCT-API), the one change increased from INFO to SEVERE, which seems reasonable. However, another project (findbugs) \emph{reduced} the log level within catch blocks. We found two such changes, from SEVERE to WARNING and SEVERE to INFO\@. After further investigation, the developers altered their view regarding the severity of the exception being caught. This latter case would be potentially problematic in this situation, however, out of 36 observed, we only found 2 such instances.

% While evaluating \guava,\footnote{This result is from an earlier tool version where heuristics were being formulated.} we had to make one manual change to the unit test code: \javainline{assertEquals(Level.INFO, record.getLevel())}. Here, a log level was actually being tested. In this case, our tool transformed the tested log level to \ji{FINEST}, which failed the test suite. While more sophisticated analysis would be required to automatically handle such cases, we conjecture such cases are rare and only found one such case during our experiments.

% % May want to discuss how we found the tool mimicking some of the human changes \url{https://github.com/eclipse/californium/pull/933#issuecomment-484638374}.

% % There was a case in \blueocean\ where our transformation worked really well by increasing a log level appearing within a catch block from INFO to SEVERE\@:

% % \begin{javacode}
% % diff --git a/blueocean-github-pipeline/src/main/java/io/jenkins/blueocean/blueocean_github_pipeline/GithubServerContainer.java b/blueocean-github-pipeline/src/main/java/io/jenkins/blueocean/blueocean_github_pipeline/GithubServerContainer.java
% % index 7f3b9a031..86c9d54e9 100644
% % --- a/blueocean-github-pipeline/src/main/java/io/jenkins/blueocean/blueocean_github_pipeline/GithubServerContainer.java
% % +++ b/blueocean-github-pipeline/src/main/java/io/jenkins/blueocean/blueocean_github_pipeline/GithubServerContainer.java
% % @@ -103,7 +103,7 @@ public class GithubServerContainer extends ScmServerEndpointContainer {
% %                          isGithubCloud = code == 200 && responseBody.containsKey("current_user_url");
% %                          isGithubEnterprise = code == 401 && responseBody.containsKey("message");
% %                      } catch (IOException ioe) {
% % -                        LOGGER.log(Level.INFO, "Could not parse response body from Github");
% % +                        LOGGER.log(Level.SEVERE, "Could not parse response body from Github");
% %                      }
% % \end{javacode}

% % Also in \blueocean, there was a case where our if condition heuristic, which did not lower levels appearing in if statements did not work so well:

% % \begin{javacode}
% % diff --git a/blueocean-git-pipeline/src/test/java/io/jenkins/blueocean/blueocean_git_pipeline/GitReadSaveTest.java b/blueocean-git-pipeline/src/test/java/io/jenkins/blueocean/blueocean_git_pipeline/GitReadSaveTest.java
% % index b300b210a..b58aee8bd 100644
% % --- a/blueocean-git-pipeline/src/test/java/io/jenkins/blueocean/blueocean_git_pipeline/GitReadSaveTest.java
% % +++ b/blueocean-git-pipeline/src/test/java/io/jenkins/blueocean/blueocean_git_pipeline/GitReadSaveTest.java
% % @@ -183,7 +183,7 @@ public class GitReadSaveTest extends PipelineBaseTest {
% %          if (sshd != null) {
% %              String ssh = "ssh -p " + sshd.getPort() + " bob@127.0.0.1";
% %              String remote = "ssh://bob@127.0.0.1:" + sshd.getPort() + "" + repoForSSH.getRoot().getCanonicalPath();
% % -            logger.fine(ssh + " // remote: " + remote);
% % +            logger.finest(ssh + " // remote: " + remote);
% %              sshd.stop();
% %              sshd = null;
% %          }
% % \end{javacode}

% % TODO:
% % Discuss \url{https://github.com/eclipse/californium/pull/933#issuecomment-487458686}:

% % \begin{quote}

% % A project with history, as californium, has many parts without too many changes even over many months. I'm not sure if this results in proper assumptions about the logging level. So in my opinion, there should be tags (annotation?) to exclude some methods, classes, and packages from such an automatic log level adjustment.

% % \end{quote}

% The following transformation took place in \selenium, a popular web application testing application. Here, a log is issued before an exception throw indicating a failure. The level \javainline{INFO} was originally used in the logging statement. This transformation was actually accepted as part of our pull request study (\cref{sec:pulls}),\footnote{Pull request URLs have been omitted to preserve author anonymity in this version.} demonstrating that although our approach is focused on event logging/feature correlations, it may also be useful in identifying mismatches due to situational severity:
% % TODO: Should add? \cite{pr-for-selenium-new}

% \begin{diffcode*}{fontsize=\footnotesize,linenos=false}
% if (!check.isAlive()) {
% -   LOG.info("Node is not alive: " + check.getMessage());
% +   LOG.severe("Node is not alive: " + check.getMessage());
% 	// Throw an exception to force another check sooner.
% 	throw new UnsupportedOperationException(
% 		"Node cannot be registered");
% }
% \end{diffcode*}

% % \begin{listing}
% % 	\begin{minted}[fontsize=\scriptsize]{diff}
% % 		  } catch (CouldNotResolveImportException e) {
% % 		- 	 logger.log(FINE, "Failure to resolve import", e);
% % 		+ 	 logger.log(WARNING, "Failure to resolve import", e);
% % 		  	 return Optional.absent();
% % 		  }
% % 	\end{minted}
% % 	\caption{A transformation for \errorp.}\label{lst:errorprone}
% % \end{listing}
% %
% % The logging statement in \cref{lst:errorprone} is enclosed by a catch block. Its log message is used to denote an error if the exception is thrown. However, level \javainline{FINE} provides tracing information, which is low for this case.

% % One project, namely,
% \CoreNLP\ included an unusual pattern where logs would consist of two statements, one for a high-level overview of the event and another that includes details of the event. While our heuristics worked for the high-level logging statement, they failed for the detailed one.
% % as it did not include the typical keywords found in logging statement classes.
% The following portrays an example of an incorrect transformation issued by our approach. Such incorrect transformations would have been avoided had a string concatenation operation been used rather than two related logging statements to describe a single event:

% \begin{diffcode*}{linenos=false,fontsize=\footnotesize}
%   ExtractionObject o = entityMap.get(arg.getContent().getId());
%   if (o == null) {
% 	  logger.severe("READER ERROR: Failed to find relation argument"
% 	      + " with id " + arg.getContent().getId());
% -     logger.severe("This happens because a few relation mentions"
% -         + " illegally span multiple sentences. Will ignore this"
% -         + " mention.");
% +     logger.fine("This happens because a few relation mentions"
% +         + " illegally span multiple sentences. Will ignore this"
% +         + " mention.");
% \end{diffcode*}

% % TODO: Should this be added? Have to anonymize PR citation.
% % After our tool was applied to \jenkins, a popular continuous integration (CI) system, ``[s]everal log messages that exist to inform admins about the state of Jenkins have been demoted from the visible-by-default \javainline{INFO} to \javainline{FINE} or \javainline{FINER}''~\cite{Beck2019}. This shows that there may be, in some cases, a disconnect between events that developers find ``interesting'' at a given time and that of particular users. Because of the highly distributed nature of \jenkins\ as a server-side software product, logging statements primary help administrators to inform them about the status of the system and help them troubleshoot any issues rather than providing assistance to developers in their development tasks (e.g., fixing bugs, making enhancements). In this case, one could argue that two different vectors of log levels would be required, depending on whether the system is being tested by developers or in production by users. However, we imagine scenarios existing where developers and users are both interested in the same events at the same time, e.g., those relating to new features, particularly in prototype development.

% % Some projects did not use the levels as described in the API documentation, e.g., there is a \href{http://github.com/junit-team/junit5/issues/513}{issue} for \junit\ on Github with CONFIG\@. This is a problem for some of our heuristics (settings).

% % \paragraph{Varying Git History Depth}

% % \commentYTi{This is for old version.}

% % The depth parameter may vary the quality of results produced by our tool. And, the more history used may not always produce the best results. When evaluating our tool against \selenium, we performed two different experiments, one considering the entire life of the project ($\approx$24,000 commits) and a much more recent set of changes (last 1,000 commits). The transformations produced in the two cases were similar except for several key differences. Using 1,000 as our threshold, our tool was able to find a log statement associated with an exception that was originally at the \javainline{INFO} level but ended at \javainline{SEVERE}:

% % \begin{javacode}
% % diff --git a/java/server/src/org/openqa/selenium/grid/node/httpd/NodeServer.java b/java/server/src/org/openqa/selenium/grid/node/httpd/NodeServer.java
% % index 732433d..121c8a6 100644
% % --- a/java/server/src/org/openqa/selenium/grid/node/httpd/NodeServer.java
% % +++ b/java/server/src/org/openqa/selenium/grid/node/httpd/NodeServer.java
% % @@ -143,7 +143,7 @@ public Executable configure(String... args) {
% % () -> {
% % 	HealthCheck.Result check = node.getHealthCheck().check();
% % 	if (!check.isAlive()) {
% % -		LOG.info("Node is not alive: " + check.getMessage());
% % +		LOG.severe("Node is not alive: " + check.getMessage());
% % 		// Throw an exception to force another check sooner.
% % 		throw new UnsupportedOperationException("Node cannot be registered");
% % 	}
% % \end{javacode}

% % This change was part of our pull request to the project~\cite{pr-for-selenium}, and we also filled an issue to alert developers of a possible inconsistency~\cite{issue-for-selenum}.

% % Also, our current approach only handles convenience methods (e.g., \javainline{logger.info(...)}) and log levels passed as literal values (e.g., \javainline{logger.log(Level.INFO,...)}). However, levels may be passed into the API via variables, and developers may wrap APIs. In either case, a more complex analysis would be necessary as multiple possible logging levels could correspond to a single logging statement. Although this an area for future work, we encountered XXX number of cases.

% % \begin{listing}
% % \begin{javacode}
% % LOGGER.log(optional ? Level.FINE : Level.WARNING,
% %   "Failed to load "+item.className(), e);
% % \end{javacode}
% % \caption{The logging statement in jenkins cannot be handled yet}
% % \end{listing}

% The following transformation took place in \jenkins:

% \begin{diffcode*}{linenos=false,fontsize=\footnotesize}
% - LOGGER.log(INFO, "{0} main build action completed: {1}",
% -     new Object[] {this, result});
% + LOGGER.log(FINEST, "{0} main build action completed: {1}",
% +     new Object[] {this, result});
% \end{diffcode*}

% \noindent This transformation was also accepted as part of our pull request study, with the developer expressing that it is ``[p]robably a good idea: [i]t's time we started removing this from the general system log \ldots.'' This indicates the feature associated with this logging statement has not been of interest to developers recently and its level should be adjusted to reflect that. This idea was reinforced in a subsequent comment for a similar transformation: ``\ldots I've grown so used to these messages over the years \ldots.''\insertrefRK{Why don't these have citations?}

% \subsubsection{Comparison With Manual Log Level Changes}

% \begin{table}
% 	\caption{Confusion matrix results for manual level change comparison.}\label{tab:confusion_matrix}
% 	\resizebox{\linewidth}{!}{%
% 		\begin{threeparttable}
% 			\begin{tabular}{lllllllll}
% 				\toprule
% 				subject & cHEAD & tHEAD & Kcmts & TP & FP & FN & \textbf{$\overline{\mathit{distR}}$} & direct\\
% 				\midrule
% 				blueocean\tnote{*} & de8b8ca & de8b8ca & 1.00 & 0 & 2 & 0 & N/A & N/A\\
% 				guava & 8385600 & 638fcb8 & 1.00 & 3 & 0 & 0 & 33.33 & 3\\
% 				IRCT-API & aa0f039 & 86d2c49 & 0.13 & 1 & 10 & 0 & 83.33 & 0\\
% 				jsilhouette & be37202 & be37202 & 0.03 & 0 & 0 & 0 & N/A & N/A\\
% 				junit5 & c7c5796 & 2fab23a & 0.47 & 4 & 15 & 4 & 25.00 & 4\\
% 				SpotBugs & 190e1e1 & 35804ee & 1.00 & 14 & 29 & 2 & 24.49 & 13\\
% 				WALA & 7f68e76 & 3317c1c & 1.00 & 1 & 0 & 0 & 50.00 & 0\\
% 				Total &  &  & 15.37 & 23 & 56 & 6 & 29.40 & 20\\
% 				\bottomrule
% 			\end{tabular}%
% 			\begin{tablenotes}
% 				\item[*] blueocean is \blueocean.
% 			\end{tablenotes}
% 		\end{threeparttable}
% 	}
% \end{table}

% % By achieving the goal of comparing the actual log level transformations with the log level transformations suggested by the tool,
% In this experiment phase, we compared the transformations produced by our tool with manual logging statement levels changes.
% % While the ultimate goal of our approach is not necessarily to mimic manual changes but rather \emph{alleviate} developers from performing widespread analysis and transformations, this phase nevertheless
% It offers additional insight into the behavior of our tool compared to manual effort. For this purpose, we mined the git histories of seven of the subjects from \cref{tab:results} (listed in \cref{tab:confusion_matrix}) and extracted actual log level changes using an automated script to construct an oracle. We manually studied the git commit messages to verify that the changes were made manually by developers (i.e., that there was no indication of any automation involved). Column \textbf{cHEAD} (\emph{c} for \emph{change}) is SHA-1 of HEAD when the extraction took place. Column \textbf{tHEAD} (\emph{t} for \emph{tool}) is the SHA-1 that the tool was run on, which was determined by selecting the earliest common commit immediately before manual log level changes. For example, if, in a particular subject, all manual changes were made in v5, tHEAD would be v4. If, on the other hand, manual changes were made in v3, v5, and v6, tHEAD would be set to v2. If there were no logging statement level changes, then $\mathbf{tHEAD}=\mathbf{cHEAD}$.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % NOTE: This confusing discussion would benefit greatly from examples.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % For each subject, we ran the tool on the earliest common SHA-1$\sim$1 (i.e., the commit immediately before SHA-1) of the git commits with log level changes to obtain the log level transformations suggested by the tool. However, for \junit\ and \spotbugs, some logging invocations could be found in the actual log level changes, but not in the earliest common SHA-1$\sim$1. They are added in the later git commits, so the tool cannot suggest log level changes for these logging invocations, which can break confusion matrix building. We observed that closed git commits of actual log level changes are always working on the same subproject. Besides, evaluation of the tool on a subproject is independent of the other subprojects in the same project. Hence, we build a confusion matrix for the projects with the issue mentioned above by analyzing their subprojects. We grouped git commits with actual changes into 10 clusters by the subprojects. Then, we run the tool on the earliest common SHA-1$\sim$1 for every cluster to get tool log level transformations. The committed time of git commits in every cluster is very close or there is only one git commit in a cluster, i.e, there is no logging invocation in git commits with actual log level changes but not in the earliest common SHA-1$\sim$1. Since one cluster is mapped to a unique subproject, no overlap of transformations suggested by the tool exists among clusters. Therefore, tool transformations for an entire project are total tool transformations for relevant clusters.

% Column \textbf{Kcmts} is then the thousands of analyzed git commits ending in \textbf{tHEAD}. In some cases, this results in a Kcmts value less than used in \cref{tab:results} since the analysis HEAD must be one that is prior to all manual changes (as explained above).

% The remaining columns of \cref{tab:confusion_matrix} denote the confusion matrix results. Column \textbf{TP} is true positives, i.e., logging statements whose levels were changed by developers that were also suggested by our tool for level transformation. Column \textbf{FP} is false positives, i.e., logging statements whose level changes were suggested by our tool but were not actually changed manually. Column \textbf{FN} is false negatives, i.e., logging statements whose levels that actually changed but were not suggested by our tool. As we were solely interested in calculating precision and recall, true negatives were not counted. The total number of logging statement levels that actually changed is equal to $\mathit{TP}+\mathit{FN}$. The overall recall ($\frac{\mathit{TP}}{\mathit{TP} + \mathit{FN}}$) is \recall\ and precision ($\frac{\mathit{TP}}{\mathit{TP} + \mathit{FP}}$) is \precision.

% Our tool considers, as input, all logging statements in a project.
% % and can suggest logging statement levels to all of them.
% However, it is tedious, time-consuming, and possibly error- and omission-prone for developers to continuously examine all logging statement levels
% % in projects and
% transform them if necessary. This is especially evident for large projects with many logging statements, as can be seen in \cref{tab:results}.
% % That's why each commit with log level changes in our experiment always focuses on one subproject, even for one or two class files.
% Therefore, a precision of \precision\ may not be indicative of \emph{all} logging statement levels that \emph{should} change as developers may have manually omitted level changes inadvertently.

% The counts in the TP column do not consider the target level, i.e., the target level chosen manually and by our tool. To account for target levels, column \textbf{$\overline{\mathit{distR}}$} depicts the average transformation distance ratio, which is computed for every log level transformation counted as a true positive. This value is the distance between the actual target log level and the target log level suggested by the tool divided by the total number of possible log levels considered for transformations.
% % The number of possible levels depends on the logging framework and settings.
% The smaller the distance ratio, the closer our tool was able to suggest similar target levels that were made manually. The average distance ratio during our experiment was \num{29.40}. However, we are also interested in knowing not only the exact target level of the suggestion compared to the actual change but also how the \emph{direction} of the transformations compared. Understanding how the tool behaves regarding the direction of the suggested transformations is arguably more important than hitting the exact target level. The two columns combined present a clear picture of the performance of the tool in terms of its ability to suggest accurate level adjustments.

% As such, column \textbf{direct} portrays level direction matching. It represents the number of true positives that had the same transformation direction (i.e., either lowering or raising) for both manual level changes and suggested level transformations.
% % Since log levels have orderings, log levels could be lowered or raised for transformations.
% In other words, if a logging statement level is lowered both manually and by the tool, it is counted as level direction match. Likewise, a match is also counted if it is both manually raised and raised by the tool. All other combinations are not counted. On average, our tool suggested transformations in the same direction as manual changes \levelDirectionSuccessRate\ ($\nicefrac{20}{23}$) of the time. 

% % \todo{Should we discuss TN?}

% % \subsubsection{Discussion}

% % It could be that there are so many conversions to FINEST because that is where most of the ``mismatches'' are coming from.

% \subsubsection{Pull Request Study}\label{sec:pulls}

% % Assessing the usefulness of our approach through pull requests, although insightful, has its challenges for program transformation. Particularly, it has been shown that developers cannot always estimate the impact of a transformation~\cite{Palomba2014}. Furthermore, developers generally perceive refactorings and other transformations as a fault-prone activity~\cite{Bavota2012,Habchi2019,Kim2014}. As such, developers may not accurately decipher the value of the presented transformations immediately. Still, we performed this assessment but only as a part of our overall evaluation.

% To assess our approach's usability, we also submitted
% % several
% pull requests (patches) containing the results of our tool to subject projects.\footnote{An early PR study on an earlier tool version was used to obtain heuristics (q.v.~\cref{sec:heuristics}).} As of this writing, eighteen requests have been made, twelve of which are currently pending, two merged (accepted), and four rejected. The two projects where our results were integrated were \jenkins\ and \selenium.
% % One of our merged \href{https://github.com/jenkinsci/jenkins/pull/4345}{pull request} is for \jenkins\@.
% \jenkins\ is a popular continuous integration (CI) engine, having $\sim$15K stars and $\sim$6.1K forks on GitHub, as of this writing.
% % Another merged \href{https://github.com/SeleniumHQ/selenium/pull/7737}{pull request} is for \selenium\ which is a popular umbrella project.
% \selenium\ is a popular web application testing and automation tool, having $\sim$17K stars and $\sim$5.6K forks.

% Apparent during our pull request study was that our approach forces developers to actively think about how their logging statement levels evolve along with their software. Using GitHub's line-by-line comment tool, developers often commented on many individual transformations. Some feedback received during the study indicated that long periods of time passed before considering altering logging statement levels (q.v.~\cref{sec:qual}).

% Feedback from rejected pull requests include thoughts on whether or not our approach is applicable to very mature and largely stable projects that are in ``maintenance mode.''
% % (\url{https://github.com/google/guava/pull/3435#issuecomment-480320723}).
% % It may be possible to guess when this situation happens by seeing that all the DOI values of logging statements are 0. Thus, our approach may not be amenable to large, mature projects, particularly frameworks, that are well-vetted and in maintenance mode.
% The problem is that, in this scenario, most likely, developers will be responding to bug reports from users, which may result in developers \emph{consistently} changing \emph{different} parts of the system. In this case, our approach will never pick more ``interesting'' parts of the system as they are all equally (not) ``interesting.'' Application/system code that is under more active development may be more amenable.
% % The problem is that the interestingness converges over time.
% Projects using sprints ala agile methods may benefit more from the approach.
% % It may not work for ``stable'' code (see \url{https://github.com/SeleniumHQ/selenium/pull/7170#issuecomment-542742545}).

% A question was also raised regarding the approach's applicability to library vs.~application code.
% % ~\addrefRK. % https://github.com/google/guava/pull/3713/files#r348532243 chktex 13
% Particularly, parts of a library that are important to library developers may not match the interest level of application developers using the library. This seems to touch on a broader issue of log composition, i.e., the log intentions of application developers may not coincide with the application's dependencies in general. This problem may be more apparent in library components that are exposed to application developers.
% % TODO: What about users; do they use the logs?

% \todoRKi{Add a discussion section before threats to validity?}

% \subsection{Threats to Validity}

% The subjects may not be representative of real-world logging statement usage. To mitigate this, subjects were chosen from diverse domains as well as sizes, as well as those used in previous studies (e.g.,~\cite{Khatchadourian2019,Ketkar2019}). Although \jdp~is artificial, it is a reference implementation similar to that of JHotDraw, which has been studied extensively (e.g.,~\cite{Marin2007}).

% The git commit history may be too course-grained with very large commits. In this case, our approach may not  be able to detect changes to program elements properly. This can occur when projects are imported into git from another repository, for example. This is a limitation of many approaches that mine version control history. Furthermore, our keyword related heuristics cannot work with typos, i.e., if a log message contains the keyword with a spelling mistake, our tool cannot detect the keyword.
% % This limitation is also indicative of many approaches that use keywords.
% Even still, there were \num{2003} logging statements in our experiments whose logging levels were not altered due to keywords, suggesting that typos are not pervasive. This threat may be mitigated by expanding the keyword set to include common misspellings, which we plan for future work.

% % Our current implementation focusing on logging statements, i.e., direct invocations to the standard Java logging API\@. The reason is is that we are interested in the relevance of the system portion immediately related to the logging statement. We could have focused instead on the logging level, however, that may not lead us directly to where to the logging statement.

% % Projects may use different APIs for logging, which we hope to include in the near future. Doing so would be straight-forward. Nevertheless, the XXX subjects we describe in Table XXX all use the standard API, which shows that our approach is still useful and applicable.

% % The limitation regarding only using the enclosing method's DOI can be problematic for large methods. Specifically, if a mismatch is found, our tool will transform each logging statement within the entire enclosing method to have the same level (except for catch blocks if that setting is enabled). Although seemingly problematic for large methods, we found instances where the logging levels were \emph{originally} the same for the entire method, e.g., \url{https://github.com/hms-dbmi/IRCT-API/pull/43/files#diff-ecd57284addd124f7e3b4d19120b967b}.

% % We notice that some log levels are transformed into FINEST\@. Most of them have an enclosing method with DOI value 0. The reason is that their enclosing methods may not be modified or rarely modified after their creation. Their DOI values become 0 eventually because of DOI value decay.\todo[inline]{RK\@: Why is this a threat to validity? This is more results discussion.}

% % Heavy refactorings that focus on one area of the system could throw off our approach, but refactorings are typically widespread. Such changes should have a minimal effect on our approach as a focal point will be more difficult to identify.

% % What if we don't go back far enough in time where the file containing the log is changed? I think things have a default DOI of 0. I guess it's what have you done for me lately, so perhaps we can argue that they should be 0.


% Lastly, code proximity may not be the correct indicator for identifying logging statements related to a software feature. Other semantic-based information, such as variable references, for example, may be more useful. However, our current results are still promising, and we plan to explore the use of semantic information for future work.


==> impl.tex <==
\section{Implementation}\label{sec:impl}

\commentRK{Does this section answer the question, ``how the tool is used?''}

\commentRK{Where are all of the comments we had in the conference paper that say ``this is good to discuss in the tool paper?'' Were those discussed?}

% Our tool is implemented as an open source Eclipse IDE~\cite{EclipseFoundation2020a} plug-in available at \url{http://git.io/fjlTY}. \commentRK{Why did we use Eclipse? Why not IntelliJ?} It is built upon JGit~\cite{EclipseFoundation2020b} and Mylyn~\cite{EclipseFoundation2020}. Eclipse is leveraged for its extensive source-to-source transformation support~\cite{Baeumer2001} and that it is completely open-source for all Java development.\todoRK{Footnote about IntelliJ here.} It also supports popular build systems, so that our plug-in may be applied to projects that use different IDEs. JGit is used for git commit extraction and Mylyn for manipulating and querying a DOI model. For transformation, Eclipse ASTs with source symbol bindings are used as an intermediate program representation. Two popular logging frameworks, namely, \javainline{java.util.logging} (JUL)~\cite{Oracle2018b} and SLF4J~\cite{QOS.ch2019}, are currently supported. However, our implementation can be extended to include others.\commentRK{This paragraph is mainly plagiarized, like many others.}
%Heuristics (\cref{sec:heuristics}) are presented as a series of tool options.

Our tool \textsc{Rejuvenate Log Levels} is implemented as an open-source Eclipse IDE~\cite{EclipseFoundation2020a} plug-in available at \url{http://git.io/fjlTY}. Eclipse IDE has been chosen for its well-documented, and well-integrated transformation support~\cite{Baeumer2001}
%, including Eclipse ASTs for an intermediate program representation. 
Eclipse provides some useful plug-ins to help development. Our tool is built upon two existing Eclipse plug-ins. It extends JGit for git history extraction and Mylyn for DOI model manipulation. Eclipse is mature and open-source platform that attracts a large number of users. They can easily download and use our plug-in for free.

\subsection{Tool Workflow}

% \begin{figure}
% 	\includegraphics[scale=0.5]{workflow}
% 	\caption{Tool workflow.}\label{fig:workflow}
% \end{figure}

\Cref{fig:workflow} presents high-level workflow for our tool. The input to our tool is Java projects (step 1). %Developers can right-click on the select projects to run the tool, then select the ``Rejuvenate log levels'' option under the menu of ``Refactor\replaced[id=RK, comment={Punctuation goes inside the quotes.}]{.''}{''.} This option can also be found in ``Quick Access''.
\commentRK{This text has nothing to do with the referenced figure. Why is this paper so different from the one \url{https://bit.ly/3cqhuPN}?}
%Next, a list of tool options which could affect transformation results are shown to developers. 
Next, a list of tool settings (step 2) is shown to users. 
%\Cref{fig:screenshot} shows the screenshot of the wizard including all settings, an option for history traversing and an input field for the maximum number of analyzed commits. The main purpose of the settings is to help identify the kinds of transformations that may yield useful results. 
%At the top of the screenshot, developers can choose the level log style, i.e., they can choose to treat particular levels as log categories. The particular levels depend on the logging framework used in our implementation. 
The settings improves the transformation quality for a specific situation where the developers' ``interestingness'' only has a little influence on the log level. Developers could try different settings to produce different transformations.


%The option ``Traverse git history to rejuvenate log levels'' is mandatory.
\commentRK{Is there a figure with the tool settings? Perhaps a screenshot of the wizard?} 

\begin{figure}
	\centering
    \includegraphics[width=\linewidth]{screenshot}
	\caption{Screenshot of the wizard for \textsc{Rejuvenate Logging Statement Levels}.}\label{fig:screenshot}
\end{figure}

%Without checking it, the tool cannot read any Git histories.\commentRK{Why?} For the rest of settings (discussed later\commentRK{Where?}), developers could try different option value sets to produce different transformations. Developers can input the number of maximum analyzed commits to reduce the analysis time. In addition, they can limit the maximum transformation distance if the transformations are too drastic, such as from \javainline{SEVERE} to \javainline{FINEST}.
\commentRK{These settings should be listed and \emph{then} described.}

\Cref{fig:screenshot} is a screenshot of the tool wizard. It shows a list of settings that developers could choose to find the appropriate transformations. The settings are described below:

\begin{enumerate}

    \item Treat particular levels as log \emph{categories}. A developer could choose \textsc{CONFIG},\textsc{WARNING} and \textsc{SEVERE} as log \emph{categories}. If a developer does this, the logging level transformations will not be applied to these logs.

    \item Never \emph{lower} the logging levels:%\label{itm:lower}

        \begin{enumerate}

        \item being in catch blocks.%\label{itm:catch}

        \item immediately following branch, such as if, else, and switch.%\label{itm:followingifs}

        \item \emph{having} particular keywords in log messages.%\label{itm:withkeys}

        \end{enumerate}

    \item Never \emph{change} the change logging levels if it immediately follows branches with condition containing a log level.%\label{itm:wrapping}

    \item Never \emph{raise} the logging level \emph{without} particular keywords in their log messages.%\label{itm:withoutkeys}

    \item Only \emph{consistently} transform the level of logging statements appearing in overriding methods.%\label{itm:subtyping}

    \item Only transform the level of logging statements up to a transformation distance threshold.%\label{itm:threshold}

\end{enumerate}

After performing the analysis, the tool may generate an error report (step 4). If there is no error, the tool can present a preview of transformations for log levels (step 5). Our tool can support the developers to choose the transformations at file level. Then, developers can let the tool make the transformations (step 6).\commentRK{This figure is too related to the one in the other paper. In fact, I would say its plagiarized. I much rather see the \emph{unique} aspects of the tool, particular its many settings and how those settings affect the transformation.}

\subsection{Architecture \& Dependencies}

\begin{figure}
    \includegraphics[width=\linewidth]{architecture}
    \caption{Software Architecture for \textsc{Rejuvenate Logging Statement Levels}.}\label{fig:arch}
\end{figure}

\commentRK{Seems strange to have a plug-in group for just one plug-in (JGit) in \cref{fig:arch}.}

\commentRK{The image \emph{sources} should be in the graphics directory. I should see two~.drawio files there corresponding to these figures.}

\Cref{fig:arch} depicts the three-layers software architecture of the tool. The top layer is the user interface that users only interact with. The middle layer is the core of the tool. The internal plugins are built based on two existing Eclipse plug-ins: JGit plug-in and Mylyn-Plugin. The internal Plug-ins are used to transform log levels by mining Git histories and manipulating a DOI model. For example, we enable a plug-in named \emph{mylyngit core} that extends Mylyn Plug-in to manipulate a DOI model and \emph{JGit} to mine Git histories. The \emph{mylyngit core} automatically makes an interaction event for each method change in Git histories, thus, it can manipulate DOI values by calling \javainline{processInteractionEvent(Object object, Kind eventKind, String origin, IInteractionContext context)} method. The \emph{mylyngit core} deals with Eclipse ASTs to locate methods. The \emph{log core} is another plugin in internal plugin-ins that is used to provide logging analysis and log level transformations. Eclipse ASTs are also processed in this plug-in for many purposes, including log level detection, method extraction, etc. The bottom layer is a framework that is composed of the framework of the application.
% in two categories which are internal plug-ins (those not interacting with users) and user-facing plug-ins (those directly interacting with users). Internal plug-ins category is the main category that is composed of two original plug-ins (\emph{mylyngit core} and \emph{log core}) made by us. We enable \emph{mylyngit core} plug-in\commentRK{Is this our plug-in? Did we make it or did we reuse it?} extends Mylyn Plug-ins to manipulate DOI values for methods and \emph{JGit} to handle Git histories. The \emph{mylyngit core} automatically makes an interaction event for each method change in Git histories, thus, it can manipulate DOI values by calling \javainline{processInteractionEvent(Object object, Kind eventKind, String origin, IInteractionContext context)} method. The \emph{mylyngit core} deals with Eclipse ASTs to locate methods. The \emph{log core} is used to provide logging analysis and log level transformations. Eclipse ASTs are also processed in this plug-in for many purposes, including log level detection, method extraction, etc. These two plug-ins are not accessible by users. The \emph{UI} plug-in provides a user-friendly UI to users so that the users without refactoring experience can easily this tool. 



%The \emph{evaluation} can print some statistical data during a transformation but prevent \emph{log core} from making any change in source code\commentRK{What?}. These statistical data are used for research only, which are not needed by most of users. Users can choose not to use this \emph{evaluation} plug-in.
\commentRK{As discussed, this isn't very interesting for this plug-in. More discussion on the extensions and dependencies would be better. Right now, there's only a single sentence.}

\commentRK{There's nothing more to be said about the tool? What happened to all of those comments about the tool paper in the conference paper?}

\subsection{Techinical Details}

% We provide an automated transformation tool for log level rejuvenation. The tool extends JGit and Mylyn to manipulate DOI model via git history.


%that programmatically manipulates a Mylyn DOI model~\cite{Kersten2005} using git histories to evolve event logging statement levels to better align with the current software features of interest.\commentRK{How is all of this related to \cref{fig:arch}?} The tool extends JGit and Mylyn to manipulate DOI model via git history.

We discuss some techinical details for our tool implementation in this section. We extract a sequence of method changes from Git Histories by JGit and Eclipse ASTs.
We use a method signature to identify a method. However, some methods may experience method renaming, or class renaming, alike, which cause the changing of method signatures. We built a renaming data structure to store historical method signature changes for all historical methods. After that, we made a hash table of mappings a method signature and its ``new'' signature using the renaming data structure to improve the performance of rename lookups. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTE: This can be for the tool paper:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We build a hash table of mappings a method signature and its ``new'' signature using this tree from the method renaming tree to improve the performance of rename lookups.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Since Mylyn computes DOI values from Mylyn interaction events recording the interactions between developers and program elements, it cannot directly produce DOI values given git histories. Our tool converts each method change in git histories to an interaction event in Mylyn task context with kind EDIT sequentially. Then, Mylyn could automatically compute DOI values for methods after conversions. We only consider interaction event kind EDIT, because git Histories cannot store the other interaction kinds, such as element selection by clicking.

In our tool implementation, DOI values of methods are determined by how developers frequently and recently edit methods. The DOI value of a method will be decreased if the developer does not edit the method for a while. The decreased rate of DOI values is controlled by Mylyn decay rate. We found that the original Mylyn decay rate is too rapidly which cause almost all of methods to have a DOI value representing the uninterestingness of developers, thus, almost all log levels are suggested to the lowest log level, such as \ji{FINEST} in JUL in our initial experiment, bringing about too many drastic transformations. As such, we had to reduce the original Mylyn decay rate to mitigate the transformations.
%We found that the original Mylyn decay rate is too rapidly which generates too many drastic transformations in our initial experiment. As such, we had to reduce the original Mylyn decay rate to mitigate the transformations.
\commentRK{This sounds too much like my comments. This is where you want more detail. This part is interesting but it is not sufficient just to copy my comments. Again, those are not meant to be published but rather expanded upon.}


\commentRK{Below is another interesting technical detail that wasn't discussed.}
\commentYT{I cannot add this for room limitation.}
Mylyn treats nonnegative DOI values as ``uninterestingness''. The DOI values of some methods may experience a long time of decreasing due to the Mylyn decay rate, their DOI values may become negative. Since all nonpositive DOI values are treated as the same by Mylyn, our tool regards these negative DOI values as 0. Therefore, the minimum of DOI values of methods is 0.

Mylyn treats negative DOI values as uninteresting. The view ``Focus on Active Task'' in Eclipse only shows elements with positive DOI values. The elements with negative DOI values are treated the same by Mylyn. Our tool could produce negative DOI values. If an element in active context are not accessed indirectly or directly for a long time, it will experience multiple times of decay and its DOI values could become negative. Thus, our processing regards negative DOI values as 0. The minimum DOI value is 0.

% See issue here: https://github.com/ponder-lab/Logging-Level-Evolution-Plugin/issues/111



%We use this model to track the ``interest'' of code elements surrounding logging statements to find \emph{mismatches}between log levels and feature interests for certain kinds of logging statements. The ``interest'' of code elements are denoted by DOI values from Mylyn.

%Furthermore, to aggregate interest levels across a development team, edits are extracted from git histories rather than from interactions with the IDE\@. The DOI model is then programmatically manipulated using the extracted edits. 

%The final model is then partitioned and compared to current logging statement levels. If a mismatch is found, the level is transformed in the source code. 

% This activity of the work presented here can also be used as a more general Mylyn utility to incorporate VCS information into the Mylyn context and actually solves \href{https://bugs.eclipse.org/bugs/show_bug.cgi?id=433030}{this bug}. That bug, though, only considers adding a single commit (diff) to the Mylyn context (also see \url{https://www.eclipse.org/forums/index.php/t/699154/}). Here, however, we create ``interaction events'' out of a \emph{history} of commits in the project.

Transformation decisions are made by the mappings between DOI value partitions and log levels. The partitions for DOI values are created by subtracting the highest DOI value in the model by the lowest and dividing the result by the number of different logging levels the logging framework provides. This calculation produces the partition DOI range size. 
%Then, each DOI range is associated with the level by order. For example, the least logging level (e.g., \ji{FINEST}) is associated with the first partition (e.g., with DOI range $[0,2.54)$). However, one of the heuristics (q.v.~\cref{sec:heuristics}) allows developers to choose whether or not to consider particular levels (e.g., they may choose to treat \ji{WARNING} and \ji{SEVERE} as kinds of log \emph{categories} rather than levels), and this can influence the partitioning scheme. In such cases, certain partitions will purposely not cause mismatches to be detected, thus affecting the transformations performed. Once the partitions have been formed, potential mismatches are discovered (step 7) by comparing the partitions with the current logging statement levels from step 2. % FIXME: How is surrounding code identified? chktex 9
%If a mismatch is found, the statement is considered for potential transformation subject to the heuristics outlined next.

% Log level transformations are guided by a set of tool settings.\commentRK{This sounds repeated.} The main purpose of the settings is to help identify the kinds of transformations that may yield useful results, e.g., Never lower the level of logging statements appearing within catch blocks. Users can choose the settings to compare different transformations.\commentRK{This is a great screenshot opportunity here to discuss the tool settings. In fact, I think we even have such a screenshot on our GitHub page. Discussing these via a screenshot from a developer's point-of-view would be a great way to differentiate from the conference paper, where we only briefly discussed them.}
% The options utilized include the following:

% \begin{enumerate}

% 	\item Treat particular levels as log categories.\label{itm:CWS}

% 	\item Never lower the level of logging statements appearing within catch blocks.\label{itm:catch}

% 	\item Never lower the level of logging statements immediately following if statements.\footnote{\mintinline[fontsize=auto]{java}{else} is treated similarity.}\label{itm:followingifs}

% 	\item Never change the level of logging statements immediately following if statements whose if condition contains a log level.\label{itm:wrapping}

% 	\item Never lower the level of logging statements \emph{having} particular keywords in their log messages.\label{itm:withkeys}

% 	\item Never raise the level of logging statements \emph{without} particular keywords in their log messages.\label{itm:withoutkeys}

% 	\item Only consistently transform the level of logging statements appearing in overriding methods.\label{itm:subtyping}

% 	\item Only transform the level of logging statements up to a transformation distance threshold.\label{itm:threshold}

% \end{enumerate}

% For~\cref{itm:CWS}, a developer may choose to treat \ji{WARNING} and \ji{SEVERE}\footnote{These levels vary depending on the logging framework used in our implementation.} as logging statement categories rather than traditional levels. This way, developers can denote that logging statements with such levels have special semantics other than a sliding scale. 

%Discuss how we had to alter the original Mylyn decay rate. Mylyn was not originally designed to handle the significant number of typical changes produced in git repositories. Instead, it was originally designed to track changes to the IDE by a single developer. As such, we found that elements in the DOI decayed too rapidly due to the vast amount of input produced by git repository mining.

\commentRK{Why aren't the below comments included? These are the interesting and unique aspects of this tool.}

\commentRK{Even this one talks about analysis challenges.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTE: This can be for the tool paper:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Multiple projects}

There is an engineering challenge regarding subprojects and git repositories.

For multiple projects, we treat each of them as an independent project and process them sequentially. The task context is cleared after each processing. For every project, we need to traverse its git history, so some Git history in a repository with multiple subprojects may be analyzed more than one time. For eliminating duplicate analysis, memoization is used here. Each time analyzing a project, we store some intermediate data, such as method changes. At the same running time, if the tool analyzes a project with the same repository, it will read the stored data directly. Thus, repository is only processed once for every running time of the tool.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\commentRK{This text seems out of place. It doesn't flow. We need to tell a story.} %While evaluating multiple projects, we let the tool treat each of them as an independent project and process them sequentially. Due to decay rate in Mylyn, we do not expect the historical methods in other projects could affect the analyzed project. The task context is not reused and cleared after each evaluation. For improving performance, we use memoization to cache the intermediate data for analyzed Git repositories. In the same running time, if the tool analyzes a project with the same repository, it will not evaluate Git histories again, i.e., the tool can use these intermediate data directly.

Our tool can evaluate multiple projects in one running time. The tool treats each of projects as an independent project and processes them sequentially. We do not expect the historical methods in other projects could affect the analyzed project due to decay rate in Mylyn. Since we use memoization to cache the intermediate data for analyzed Git repositories for improving performance, the tool can save a lot of evaluation time if it evaluates multiple projects in one repository. 

Currently, our tool cannot detect log levels if levels are stored in variables. %While using the data-flow analysis to more accurately extract these levels is a subject of future work, despite this limitation, our tool is able to detect almost all log levels because these log levels are a tiny fraction of log levels in the real world. 
However, according to the data from our experiment on \logs~logging statements, only \analyzedPercentageNon~log levels belongs to this kind. We can use data-flow analysis to more accturate log level extraction in the future. In addition, the current limitation is manual Mylyn task creation and activation, which should be automated in the future.
%Since log level transformations require a valid Git repository of the analyzed project, we are unable to use a test suite by unit tests. Instead, we made a small repository for manual tests. Each branch is for one test case.

\commentRK{As previously discussed, what about the limitation where the developer has to manually create a fake task for the tool to work? Was that fixed? If not, it should be discussed with possible ways to fix it in the future.}

% \subsection{Software Analysis Challenges}

\commentRK{This is not the intent of this requirement. The analysis challenges are that of the developer's using our tool not of the tool itself: ``
the software analysis challenge(s) the tool \textbf{addresses}.} % chktex 36

% Since our tool provides several settings, developers may hesitate at choosing setting combinations. They can try different settings, but it should take time. Besides, our tool does not help developers test whether their code has obvious faults. Instead, it may indirectly affect testing, because logs can convey information in a more effective way after our log level transformation.

% Currently, our tool cannot detect log levels if levels are stored in variables. While using data-flow analysis to more accurately extract these levels is a subject of future work, despite this limitation, our tool is able to detect almost all log levels because these log levels are a tiny fraction of log levels in the real world. According to the data from our experiment on \logs~logging statements, only \analyzedPercentageNon~log levels belongs to this kind.

\commentRK{As we discussed during our meeting, our tool is not related to helping developers test their code. While the below discussion is interesting from a technical standpoint, it is not related to this requirement. This may go in as a ``technical detail.''}

% Since log level transformations require a valid Git repository of the analyzed project, we are unable to use a test suite by unit tests. Instead, we made a small repository for manual tests. Each branch is for one test case.

\subsection{How the tool is used}\label{sec:used}

\commentRK{\Cref{sec:used}, like all sections, needs a title that is in \emph{title} case.}

After successful installation via Eclipse Update Site, developers can right-click on projects for evaluating to run the tool, then select the ``Rejuvenate log levels'' option under the menu of ``Refactor''. It can also be found in ``Quick Access'' in the top-right corner of the Eclipse workspace window. Next, a wizard (\cref{fig:screenshot}) shows up. The option ``Traverse git history'' should be always selected, allowing the tool to read git history. Developers can try different settings and input the maximum number of analyzed commits in this dialog. Next, they can click ``Next'' to see a preview of transformations without any error reporting. Then, developers can click ``Next'' to apply transformations to source code. The button ``Finish'' can lead to automated transformations in source code without any preview.


==> motive.tex <==
% \section{Motivating Example}\label{sec:motiv}
\section{Software Engineering Challenges}

% Our focus is on analysis challenges. What are the analysis challenges the developers face in this domain? How does the tool help \emph{address} those challenges? This section should be modeled after \url{https://bit.ly/2zcovFz}, which was modeled after the original motivation section of the conference paper.}
Rejuvenating log levels needs subtle considerations, which also face several challenges and can be solved by our tool:

\begin{enumerate}

    \item Each logging framework provides several log levels. It may be difficult for developers to adjust log levels, because they may not well-estimate the benefit for each log level in a logging framework. Our tool can automatically rejuvenate log levels, help developers make decisions.
    
    \item As software evolves, such as new feature adds, enhancements, and bug fixes, the log level may require alternations. However, the software evolving is a continuous process, i.e., the requirements for alternations may be needed for the entire period of software evolving. Developers can transform log levels at any time by easily running our tool. 
    
    \item The number of logging statement levels may be huge, especially in the highly transactional software, it may take too much time to check all log levels. Our tool can evaluate all log levels in the analyzed projects automatically.

\end{enumerate}


% We present a multiversioned example that motivates the proposed approach and highlights some of the challenges associated with automation.
% % distinguishing different kinds of logging statements.

% \begin{listing}
% 	\begin{javacode}
% 		public class Wombat {|\label{lne:wombat}|
% 			private static final Logger logger = // A logger that only logs |$\geq$| FINE ...|\label{lne:logger}|
% 			private int temperature;|\label{lne:tempStart}|
% 			private int oldTemperature;|\label{lne:tempEnd}|

% 			public void setTemperature(int val) {|\label{lne:setTempStart}|
% 				this.oldTemperature = temperature;|\label{lne:setTemp}|
% 				this.temperature = val;|\label{lne:cache}|
% 				logger.log(Level.FINER, "Temperature set to: " + this.temperature);|\label{lne:logTemp}|
% 				logger.finer("The old temperature was: " + this.oldTemperature);|\label{lne:logOldTemp}|
% 			} // ...

% 			public static void main(String[] args) throws Exception {|\label{lne:mainStart}|
% 				Wombat w = new Wombat();|\label{lne:createWombat}|
% 				Scanner scanner = new Scanner(System.in);

% 				System.out.println("Enter a temperature:");
% 				int input = scanner.nextInt();|\label{lne:ask}|
% 				w.setTemperature(input);|\label{lne:tempSet}|

% 				try { // send to file.|\label{lne:fileStart}|
% 					logger.fine("Writing to file.");|\label{lne:fileLog}|
% 					Files.writeString(new File("output.txt").toPath(), w.toString(),|\label{lne:writeStart}|
% 						StandardOpenOption.WRITE);|\label{lne:writeEnd}|
% 				} catch (IOException e) { // Fatal error.
% 					logger.severe("Couldn't open file for writing.");|\label{lne:logError}|
% 					throw e;
% 				}|\label{lne:fileEnd}|
% 			}
% 		}
% 	\end{javacode}
% 	\caption{Logging usage example inspired by \citetitle{QOS.ch2019a}~\cite{QOS.ch2019a}.}\label{lst:wombat}
% \end{listing}

% \Cref{lst:wombat} portrays a hypothetical code snippet inspired by the \citetitle{QOS.ch2019a}~\cite{QOS.ch2019a}; it was rewritten to use JUL to demonstrate a wider spectrum of log levels, which include, in ascending order, \ji{FINEST}, \ji{FINER}, \ji{FINE}, \ji{INFO}, \ji{WARNING}, and \ji{SEVERE}. A \javainline{Wobmat} class is declared starting at line~\ref{lne:wombat} and has an available \javainline{logger} (line~\ref{lne:logger}) and a current and previous \javainline{temperature} (lines~\ref{lne:tempStart}--\ref{lne:tempEnd}). To reduce information overload (e.g., in production), the \javainline{logger} is configured so that only logs with levels $\geq$ \javainline{FINE} are emitted.

% A mutator method for \javainline{temperature} begins on line~\ref{lne:setTempStart}. Before the new \javainline{temperature} is set on line~\ref{lne:setTemp}, the old value is cached on line~\ref{lne:cache}. Then, the new temperature is logged on line~\ref{lne:logTemp} and the old is logged on line~\ref{lne:logOldTemp}.\footnote{\mintinline[fontsize=auto]{java}{Logger.finer()} is a convenience API for \mintinline[fontsize=auto]{java}{Logger.log(Level.FINER,...)}.} Both statements log at the \javainline{FINER} level; the difference is to show the different methods that can used. Since \javainline{logger} has been previously configured not to emit logs with levels $\leq$ \ji{FINER}, the statements have no effect.

% Starting on line~\ref{lne:mainStart}, a \javainline{main()} method demonstrates a usage of \javainline{Wobmat}s. In creating a \javainline{Wombat} (line~\ref{lne:createWombat}), the user is asked for a temperature (line~\ref{lne:ask}), which is then set on line~\ref{lne:tempSet}. A string representation of the \javainline{Wombat} (not shown) is then saved in a file (lines~\ref{lne:fileStart}--\ref{lne:fileEnd}). The statement at line~\ref{lne:fileLog} logs that the writing has commenced. Since the level is \ji{FINE},
% % like the logs at lines~\ref{lne:logTemp}--\ref{lne:logOldTemp},
% this statement
% % also has no effect.
% emits a log. The actual file writing takes places on lines~\ref{lne:writeStart}--\ref{lne:writeEnd}. Because \javainline{Files.writeString()} throws a possible \javainline{IOException}, the call is surrounded by a try/catch block. The statement at line~\ref{lne:logError} when an exception has been caught. Unlike the previous statements, this log message is emitted as \ji{SEVERE} $\geq$ \ji{FINE}.

% \begin{listing}
% 	\begin{diffcode}
% @@ -23,11 +23,15 @@ public void setTemperature(int val) {
% +   if (val > 0) {
% |\label{lne:guardStart}|        this.oldTemperature = temperature;
% 		this.temperature = val;
% 		logger.log(Level.FINER, "Temperature set to: " + this.temperature + ".");
% |\label{lne:guardEnd}|        logger.finer("The old temperature was: " + this.oldTemperature);
% +   } else {
% |\label{lne:except}|+       throw new IllegalArgumentException("Invalid temperature: " + val);
% +   }
% } // ...

% @@ -38,7 +42,17 @@ public static void main(String[] args) throws Exception
% 	int input = scanner.nextInt();
% |\label{lne:clientStart}|+   while (true) {
% +	   try {
% 	        w.setTemperature(input);
% +		   break; // succeeded.
% +	   } catch (IllegalArgumentException e) {
% +          // Not a fatal error. Log the exception and retry.
% |\label{lne:caught}|+          logger.log(Level.INFO, "User entered invalid input: " + input, e);
% +          System.out.println("Invalid temperature. Please retry.");
% +	   }
% |\label{lne:clientEnd}|+	}
% 	\end{diffcode}
% 	\caption{Rejecting invalid temperatures.}\label{lst:wombat2}
% \end{listing}

% \begin{listing}
% 	\begin{diffcode}
% @@ -30,6 +30,9 @@ public void setTemperature(int val) {
% 	} else {
% 		throw new IllegalArgumentException("Invalid temperature: " + val);
% 	}
% +
% +   if (((double) (this.temperature - this.oldTemperature)) / this.oldTemp > 0.05)
% |\label{lne:degrees}|+       logger.warning("Temperature has risen above 5%.");
% } // ...
% 	\end{diffcode}
% 	\caption{Warning about drastic temperature changes.}\label{lst:wombat3}
% \end{listing}

% \Cref{lst:wombat2} portrays a commit made to produce a subsequent version of \cref{lst:wombat} where invalid (negative) \ji{temperature}s are rejected.\footnote{Although the examples show only additive changes, similar issues may arise with deletions.} This is accomplished by guarding the \javainline{temperature} assignment code and log statements (lines~\ref{lne:guardStart}--\ref{lne:guardEnd}) and throwing an exception on line~\ref{lne:except}. Likewise, the client code changes to handle the exception (lines~\ref{lne:clientStart}--\ref{lne:clientEnd}), looping until proper input is received. On line~\ref{lne:caught}, a log is issued when the thrown exception is caught documenting the retry. Because the error is non-fatal, the \ji{INFO} level is used. An ensuing commit is made in \cref{lst:wombat3} so that drastic temperature changes are logged. The change is in \javainline{setTemperature()}, where a warning is logged on line~\ref{lne:degrees} if the temperature has increased above \SI{5}{\percent}.

% \begin{listing}
% 	\begin{javacode}
% 		public void setTemperature(int val) {
% 			if (val > 0) {
% 				this.oldTemperature = temperature;
% 				this.temperature = val;
% 				logger.log(Level.|\st{FINER}\smash{\ul{FINE}}|, "Temperature set to: " + this.temperature);|\label{lne:transformFine}|
% 				logger.|\st{finer}\smash{\ul{fine}}|("The old temperature was: " + this.oldTemperature);|\label{lne:transformFine2}|
% 			} else {
% 				throw new IllegalArgumentException("Invalid temperature: " + val);
% 			}

% 			if (((double) (this.temperature - this.oldTemperature)) / this.oldTemperature > 0.05)
% 				logger.warning("Temperature has risen above 5%.");|\label{lne:tempWarn}|
% 		} // ...

% 		public static void main(String[] args) throws Exception { // ...
% 			while (true) {
% 				try {
% 					w.setTemperature(input);
% 					break; // succeeded.
% 				} catch (IllegalArgumentException e) {
% 					// Not a fatal error. Log the exception and retry.
% 					logger.log(Level.INFO, "User entered invalid input: "+ input, e);|\label{lne:invalidInput}|
% 					System.out.println("Invalid temperature. Please retry.");
% 				}

% 			try { // send to file.
% 				logger.|\st{finer}\smash{\ul{finest}}|("Writing to file.");|\label{lne:fileDecrease}|
% 				Files.writeString(new File("output.txt").toPath(), w.toString(),
% 					StandardOpenOption.WRITE);
% 			} catch (IOException e) { // Fatal error.
% 				logger.severe("Couldn't open file for writing.");|\label{lne:fileError}|
% 				throw e;
% 			}
% 		}
% 	\end{javacode}
% 	\caption{Abbreviated final example with ``rejuvenated'' log levels.}\label{lst:wombat4}
% \end{listing}

% \todoRKi{May be able to shorten up \cref{lst:wombat4}.}

% \todoRKi{Is \cref{lst:wombat3} really necessary?}

% \Cref{lst:wombat4} depicts an abbreviated result, containing only relevant parts, of \cref{lst:wombat} with the commits in \cref{lst:wombat2,lst:wombat3} applied to it. Note that there are several transformations to the log levels made in the example. For instance, the levels at lines~\ref{lne:transformFine}--\ref{lne:transformFine2} have \emph{increased} from \ji{FINER} to \ji{FINE}. This is because of the recent changes made in \cref{lst:wombat2,lst:wombat3} are to the nearby code of these logging statements, indicating that perhaps the feature implemented at this part of the code, in this case, temperature management, is of a higher ``interest'' to its developers. In other words, temperature management is a feature that is under \emph{active} development, and it may be useful to show logs related to this feature more prominently to developers, i.e., by increasing their log levels. Doing so may help developers debug the new feature code, e.g., here, to reason about temperature validity and whether drastic increases in temperature invoke the proper alarms. In this particular example, these transformed logs will now emit due to the \ji{logger}'s run time log level of \ji{FINE}, possibly assisting with the development of this feature.

% In contrast to the above, the level of the logging statement at line~\ref{lne:fileDecrease} \emph{decreased} from \ji{FINE} to \ji{FINEST}. This is because the file writing feature is \emph{not} being actively developed and may not be of particular ``interest'' to developers currently. Particularly, two commits took place that did not include any edits to this region. The effect is that this log is suppressed in this configuration. While it is possible to have regressions in code not recently edited, the logging statement alerting of an exception at line~\ref{lne:fileError} did \emph{not} have its level lowered and thus remains useful in finding possible regressions. Likewise, the logging statement at line~\ref{lne:invalidInput}, although not a fatal error, was not lowered despite recent non-local edit in \cref{lst:wombat3}.

% Although only a simple example is demonstrated here, since logging is pervasive in modern (highly transactional) software, manually managing logging statement levels to combat information overload can be an overwhelming and daunting task. Even in this simple example it is easy to see that logging statements can be widespread, scattered, and tangled with code implementing core functionality. Automatically bringing event information related to software features that are developed more and more often to the forefront of developers' attention, while gradually suppressing those of features less and less frequently developed may help developers hone in their focus to catch errors during development and debugging.


==> scratch.tex <==
We help developers rejuvenate log levels in the source code to enhance logs. Developers can be able to print critical information while ignoring insignificant information through log levels. Based on the widely used Java Logging APIs we are researching on~\cite{Oracle2018}, log levels are \javainline{ALL}, \javainline{FINEST}, \javainline{FINER}, \javainline{FINE}, \javainline{CONFIG}, \javainline{INFO}, \javainline{WARNING}, \javainline{SEVERE}, \javainline{OFF}. The ordering of log levels usually reflects how developers are interested in the software parts where their log invocations are in, e.g., the software part which includes an log invocation with log level \javainline{FINEST} gains less interests from developers than the log level \javainline{INFO}. The software part is the context of a log invocation. It could be composed of some adjacent statements, enclosing block or enclosing method. Enclosing method is the method where the log invocation locates. However, there are some special cases for log levels. In this paper, we do not consider \javainline{ALL} and \javainline{OFF}, because they are used to turn on/off logging. Besides, we should consider \javainline{CONFIG}, \javainline{WARNING} and \javainline{SEVERE} carefully. \javainline{CONFIG} could be used to record static configuration information~\cite{logger}, while \javainline{WARNING} or \javainline{SEVERE} often indicates there is potential problem or a failure for program, which needs extra attention from developers. For these special log levels above, we need to consider them prudently and separately.

Developers always have challenges to evolve log levels. The previous research indicates that developers cannot well estimate cost and benefit for each log level, so they always spend much time to adjust log levels~\cite{Chen2017}. Moreover, developers always switch their interests on different software parts. At some points, developers may focus on one software part, and select a higher log levels for the log invocations in that software part. After a period of time, the software part is no longer important, but its log levels still present significance. This case always happens. \citet{Li2017}~analyzes four famous subjects and find that only 2.9\% logging statements experience level changes after their introduction. However, developers' interests always change, i.e., log levels do not always match developers' interests. They present that log levels of logging statements developers write may not be correct or may change overtime with requirements, and it is impossible to know for sure what the correct level should be. In our paper, however, we assume that more ``interesting'' parts of a software system should have, in general, higher log levels (e.g., \ji{INFO}) that less interesting parts (e.g., \ji{FINEST}). Our assumption helps developers judge the fit of log levels.

Based on our assumption, we propose an approach to help developers automatically rejuvenate log levels by using Degree Of Interests (DOI). DOI is an model which is able to provide degree of developers' interests in program elements by evaluating interaction events between developers and program elements. The model could assign a real number to an program element. That number shows the degree that developers are interested in it. That number is computed from interaction events, e.g., a developer edits an program element. DOI is a mature model and it is also implemented in Mylyn which is a Eclipse task and application life-cycle management plugin~\cite{mylynK}. Our research tries to rejuvenate log levels through matching the DOI values of their enclosing software part. However, many developers may not use, or even may not know Mylyn. We extend our theory to all git projects. We convert git differences to Mylyn interaction events so that our tool could read DOI value for the project without using Mylyn plugin. The tool could consistently make the transformations automatically based on new developers' activities.


==> scratch2.tex <==
\begin{listing}
	\begin{javacode}
	 if (logger.isLoggable(Level.SEVERE)) {
		logger.log(Level.SEVERE, message(context), exception);
	 }
	\end{javacode}
	\caption{Logging wrapping from guava}\label{lst4}
\end{listing}

We also notice some cases that need delicate consideration. In the case of Lising\ref{lst4}, the if condition has a correlation with log level, i.e., log level is determined by if condition. In this case, we should not change a log level in a logging statement.

\begin{listing}
	\begin{diffcode}
	catch (BindException e) {
		...
	-   LOGGER.log(Level.FINE, "Failed to listen to UDP port "+PORT,e);
	+   LOGGER.log(Level.WARNING, "Failed to listen to UDP port "+PORT,e);
	 }
	\end{diffcode}
	\caption{Log level changes in catch blocks from \jenkins}\label{lst5}
\end{listing}

The last case in Listing\ref{lst5} presents developers higher the log level in a catch block. \citet{Fu2014} indicates that exception types may have correlation with developers' logging decision in a catch block. In this case, we need to process them separately.



==> scratch3.tex <==


